Transient impact from the Nash equilibrium of a permanent market impact game

A large body of empirical literature has shown that market impact of financial prices is transient. However, from a theoretical standpoint, the origin of this temporary nature is still unclear. We show that an implied transient impact arises from the Nash equilibrium between a directional trader and one arbitrageur in a market impact game with fixed and permanent impact. The implied impact is the one that can be empirically inferred from the directional trader's trading profile and price reaction to order flow. Specifically, we propose two approaches to derive the functional form of the decay kernel of the Transient Impact Model, one of the most popular empirical models for transient impact, from the behaviour of the directional trader at the Nash equilibrium. The first is based on the relationship between past order flow and future price change, while in the second we solve an inverse optimal execution problem. We show that in the first approach the implied kernel is unique, while in the second case infinite solutions exist and a linear kernel can always be inferred.

==> AC_TIM_backup <==
\section{Initial Modeling}
\label{intial_setting}
%fare uno schemo del mercato primario in cui l'impatto è permanente, e poi mercato secondario ma quale decay kernel assumere?----> siccome ho simmetria allora assumo TIM, quindi il TIM è generato dalla interazione del mercato primario fra gli agenti (mercato reale e un mercato fittizzio senza competitori)

%due mercato primario e secondario--> marketi impact 



%Introduzione su market impact game di S&Z risk neutral and one asset
Our setting is characterized by two market models.
%intro generale su mercato with possible many agents and many assets
%mercato with no other competitors--uso dei market impact games per arrivare allo studio dell'equilibrio
In the first one the interactions of $J$ agents trading $M$ assets
characterize the price dynamics
through price impacts provided by the strategies of the traders.
The price dynamics is the result of the dynamical equilibrium between the activity
of agents simultaneously trading the $M$ assets.
For this setting, market impact games provide an appropriate model to derive the corresponding (Nash) equilibrium and to study how it affects the price process, see \cite{schied2018market}.
We briefly recall the market impact game framework in the next section.

In the second market model there is only one agent who determines the price impact due to his/her trading activity. In this case, the agent 
does not consider the possible presence of other competitors.
For the sake of simplicity, we refer to the two market settings as \emph{primary} and \emph{secondary market} model, respectively.
We may imagine the primary market as a better proxy of
how ``real" market impact acts, w.r.t. the secondary market, which represents instead a simple way
to describe price impact.
We summarize the two market proxies in the diagrams of Figure \ref{market_setting}.

\begin{figure}[!h]

\centering
\subfloat[][Primary Market Model]{%\label{primary}
\begin{tikzpicture}
[node distance = 1cm, auto,font=\footnotesize,
% STYLES
every node/.style={node distance=3cm},
% The comment style is used to describe the characteristics of each force
comment/.style={rectangle, inner sep= 5pt, text width=4cm, node distance=0.25cm, font=\scriptsize\sffamily},
% The force style is used to draw the forces' name
force/.style={rectangle, draw, fill=black!10, inner sep=5pt, text width=4cm, text badly centered, minimum height=1.2cm, font=\bfseries\footnotesize\sffamily}] 

% Draw forces
\node [force] (OF_M) {Order Flow Asset M};
\node [force, above of=OF_M] (agentj) {Agent J};
\node [force, left=4cm of agentj] (agent1) {Agent 1};
\node [force, left=4cm of OF_M] (OF_1) {Order Flow Asset 1};
% \node [force, right=1cm of rivalry] (users) {Bargaining power of users};
\node [force, below of=OF_M] (P_M) {Price Asset M};
\node [force, left=4cm of P_M] (P_1) {Price Asset 1};
%%%%%%%%%%%%%%%
% Change data from here



% SUBSTITUTES
% \node [comment, right=0.25 of agentj] {Interaction};
% \node [comment, right=0.25 of OF_M] {Market Impact};

% USERS
% \node [comment, below=0.25 of users] {(+) Increasing the user information\\
% (+) Reducing the switching costs};



%%%%%%%%%%%%%%%%

% Draw the links between forces
\path[->,thick] 
(agent1) edge (OF_1)
(agent1) edge (OF_M)
(agentj) edge (OF_1)
(agentj) edge (OF_M)
(OF_1) edge (P_1)
(OF_1) edge (P_M)
(OF_M) edge (P_1)
(OF_M) edge (P_M);

\path[-,thick,dashed] 
(agent1) edge (agentj)
(OF_M) edge (OF_1)
(P_M) edge (P_1);


\end{tikzpicture} }\\ \vspace{1cm}
\subfloat[][Secondary Market Model]{%\label{secondary}
\begin{tikzpicture}
[node distance = 1cm, auto,font=\footnotesize,
% STYLES
every node/.style={node distance=3cm},
% The comment style is used to describe the characteristics of each force
comment/.style={rectangle, inner sep= 5pt, text width=4cm, node distance=0.25cm, font=\scriptsize\sffamily},
% The force style is used to draw the forces' name
force/.style={rectangle, draw, fill=black!10, inner sep=5pt, text width=4cm, text badly centered, minimum height=1.2cm, font=\bfseries\footnotesize\sffamily}] 

% Draw forces
\node [force] (agent1) {Agent};
\node [force, below of=agent1] (OF_1) {Order Flow Asset 1};
\node [force, right=4cm of OF_1] (OF_M) {Order Flow Asset M};
% \node [force, right=1cm of rivalry] (users) {Bargaining power of users};
\node [force, below of=OF_M] (P_M) {Price Asset M};
\node [force, left=4cm of P_M] (P_1) {Price Asset 1};
%%%%%%%%%%%%%%%
% Change data from here



% SUBSTITUTES
% \node [comment, right=0.25 of agentj] {Interaction};
% \node [comment, right=0.25 of OF_M] {Market Impact};

% USERS
% \node [comment, below=0.25 of users] {(+) Increasing the user information\\
% (+) Reducing the switching costs};



%%%%%%%%%%%%%%%%

% Draw the links between forces
\path[->,thick] 
(agent1) edge (OF_1)
(agent1) edge (OF_M)
(OF_1) edge (P_1)
(OF_1) edge (P_M)
(OF_M) edge (P_1)
(OF_M) edge (P_M);

\path[-,thick,dashed] 
(OF_M) edge (OF_1)
(P_M) edge (P_1);


\end{tikzpicture} }
\caption{Diagrams of the two market settings.}
\label{market_setting}
\end{figure}



\begin{os}
To better clarify our contribution,
it is trivial that the secondary market is a particular case of the primary market model. From the point of view of optimal execution problem it is clear that
the solution provided by the primary market 
is indeed optimal also with respect to the secondary market, in the sense of Nash equilibrium, see e.g., Table 1 in \cite{cordoni2020instabilities}. 
The optimal execution schedule of a trader should take into account the simultaneous presence of other traders, so that agents will adopt the primary market solution. 
 Actually,
the two market proxies are redundant from the point of view of optimal execution problem. 
% It is clear that the primary market proxy represents the best way, w.r.t. the secondary market, to derive optimal liquidation strategies, since it describes a more realistic 
% market setting, where may also have many agents trading more assets, see  \cite{schied2018market}, \cite{luo_schied} and
% \cite{cordoni2020instabilities}.
However, 
we remark that this is not
the purpose of this work, which is instead to exhibit 
an evidence of transient impact by a suitable simple market setting, 
as described as follows.
To pursue this scope, we study optimal schedules provided by the two market settings.
% we do not want to find the best model to obtain the optimal liquidation strategy.
% What we want --- derivare il gisuto propagatore per il secondo market
\end{os}

In the primary market we consider a market impact game with an agent who wants to liquidate a position in an asset, that we name \emph{directional}, which interacts with $J-1$ traders who try to profit from the price impact of the other agents, named \emph{arbitrageurs}. 
Even if, recent works have highlighted how market impact games can be studied in the more general setting with $J$ risk-averse agents trading $M$ assets, (\cite{luo_schied} and \cite{cordoni2020instabilities}), we consider the simpler setting with $J=2$ risk-neutral agents trading the same asset ($M=1$) of the original framework of \cite{schied2018market}.
On the other hand, in the secondary market we consider a risk-neutral directional as the only market participant.

The two markets may differ in terms of many parameters, but we focus 
 principally on the two functions which describe the price impact.  
In other words, the two market models have the same parameters 
with an exception of the price impact function. 
% We may think the primary market 
% as a proxy for the "real" market, where all the parameters can be estimated and they represent the 
Thus, the question that we intend to 
address is the following: 
given the market impact function of the primary market, what is the related market impact function which we have to select in the secondary market so that the optimal solutions of the directional are equal for both market settings? 
 We consider the primary market as the benchmark model (from the point of view optimal execution problem),
 from which we may 
derive the related Nash equilibrium 
also for the secondary market.
In other words, we want to know if it is possible to obtain the same 
optimal solution of the primary market also in the setting of the secondary, by selecting a suitable propagator function so that we achieve the same optimal schedule.
Essentially, the selected market impact function intrinsically incorporates the interaction of agents.
The reason behind this can be motivated from the fact that we obtain the optimality 
in a simpler model, which in turn means that we have to estimate generically fewer parameters.
In particular, we want to ask the following question:
what is the market impact function that we have to select in the secondary market when in the first one the market impact is constant?
This last setting correspond to the classical Almgren-Chriss 
framework generalized with two agent. We discuss how we may use the market impact setting and Almgren-Chriss model in the next section.



% ragione avere un modello più semplice per il fund , significa stimare meno parametri  in generale , e avere lo stesso una soluzione ottimale anche rispetto a tenere conto la presenza si competitori. In particolare -AC framework per il priamry market






\section{Market Impact Games and Almgren and Chriss Model}\label{market_impact_game}
Following \cite{schied2018market}, we consider the standard framework of market impact games, i.e., 
two risk-neutral traders who want to liquidate (with inventory $X_1$ and $X_2$, respectively) the same asset during the same time interval  $0=t_0<t_1<\cdots <t_N=T$.


Given a suitable probability space 
$(\Omega,(\F_t)_{t\geq0},\F,\p)$, the price dynamics is described by a right-continuous, $S_t^0$ martingale when none of the agents trade.
However, the two traders want to unwind
 a given initial position with inventory $Z\in \R$,
 where a positive (negative) inventory means a short (long) position,
 during a given trading time grid $ \T=\{t_0,t_1,\ldots,t_N\},$ where
 $0=t_0<t_1<\cdots <t_N=T$ and following 
 an admissible strategy, which is a sequence of random variable 
 $\bm{\zeta}=(\zeta_0,\zeta_1,\ldots,\zeta_N)$ such that
 $\zeta_k \in \F_{t_k} \text{ and bounded},\  \forall k=0,1,\ldots,N$, and
 $\zeta_0+\zeta_1+\cdots+\zeta_N=Z$, see \cite{schied2018market} for further details.
The components of $\bm{\zeta}$
represent the order flow during the trading time $t_k$ for each $k=0,1,\ldots,N$.
 We denote with $X_1$ and $X_2$ the initial 
inventories of the two considered agents, with  $\Xi=(\xi_{i,k})\in \R^{2 \times (N+1)}$ the matrix 
of the respective strategies, where 
$\bm{\xi}_{1,\cdot}=\{ \xi_{1,k} \}_{k \in \numberset{T}}$
and 
$\bm{\xi}_{2,\cdot}=\{ \xi_{2,k} \}_{k \in \numberset{T}}$
are the strategies of trader $1$ and $2$, respectively.
Thus, when the two agents place orders, the price dynamics is characterized by
the permanent impact. In the 
seminal work of \cite{schied2018market}
 it is assumed the
 transient impact model of \cite{Bouchaud, BFL}, which describes the price process $S_{t}^{\Xi}$
affected by the 
strategies $\Xi$ of the two traders, i.e.,
\[
   S_t^{\Xi}= S_t^0 -\sum_{t_k <t} G(t-t_k)(\xi_{1,k}+\xi_{2,k}), 
   \quad \forall\ t \in \numberset{T},
\]
where $G:\R_{+}\to \R_+$ is the market impact function,  also called \emph{decay kernel}, describing the lagged price impact of a unit buy or sell order
over time.

The objective of the agents is to minimize their expected costs given the other traders strategies, $\E[C_{\T}(\bm{\xi}_{1,\cdot}|\bm{\xi}_{2,\cdot})]$, where the 
cost function is $C_{\T}(\bm{\xi}_{1,\cdot}|\bm{\xi}_{2,\cdot})$ is described by the sum of the permanent impact and the temporary impact modeled by a quadratic term $\theta \xi_{1,k}^2$ at trading time $k$. We refer to \cite{schied2018market} for a complete discussion on the definition of the cost functional. The temporary impact  
$\theta \xi_{j,k}^2$, for each trader$j$, 
models the slippage cost, but it 
can also be interpreted 
as quadratic transaction fee, see \cite{schied2018market}. 
In this work we adopt the mathematical modeling of Schied and Zhang 
and we do not specify exactly what this term represents.

Given the expected costs functionals of the two agents, it is straightforward to define the related Nash equilibrium.
Then, \cite{schied2018market} showed that for any strictly positive definite (in the sense of Bochner) decay kernel $G$, time grid $\T$, transaction cost parameter $\theta \geq0$, and initial inventories $X_1$, $X_2$
there exists a unique Nash equilibrium 
$(\bm{\xi}_{1,\cdot}^*,\bm{\xi}_{2,\cdot}^*)$
and it is deterministic. Moreover, it is provided by
\begin{align}\label{eq_1_S&Z}
\bm{\xi}_{1,\cdot}^*&=\frac{1}{2} (X_1 +X_2)\bm{v}
+\frac{1}{2} (X_1 -X_2)\bm{w}
\\
\label{eq_2_S&Z}
\bm{\xi}_{2,\cdot}^*&=\frac{1}{2} (X_1 +X_2)\bm{v}
-\frac{1}{2} (X_1-X_2)\bm{w},
\end{align}

where the fundamental solutions $\bm{v}$ and $\bm{w}$ are 
defined as 
$
   \bm{v}=\frac{1}{\bm{e}^T (\Gamma_{\theta}+\widetilde{\Gamma})^{-1}\bm{e}}(\Gamma_{\theta}+\widetilde{\Gamma})^{-1}\bm{e}$ and
     $\bm{w}=\frac{1}{\bm{e}^T (\Gamma_{\theta}-\widetilde{\Gamma})^{-1}\bm{e}}(\Gamma_{\theta}-\widetilde{\Gamma})^{-1}\bm{e}
$
and  $\bm{e}=(1,\ldots,1)^T \in \R^{N+1}$. 
The solutions are called fundamentals, since they 
represent the Nash equilibrium when $X_1=X_2=1$ and 
when $X_1=-X_2=1$, respectively.
The kernel matrix $\Gamma \in \R^{(N+1)\times (N+1)}$ is given by
  $
   \Gamma_{ij}=G(|t_{i-1}-t_{j-1}|), \ i,j=1,2,\ldots,N+1,
 $
 where for $\theta\geq0$ it is $
   \Gamma_{\theta}:=\Gamma+2\theta I$,   and the matrix $\widetilde{\Gamma}$ is given by
  \[
\widetilde{\Gamma}_{ij}=
  \begin{cases}
   \Gamma_{ij} & \text{ if }i>j\\
      \frac{1}{2}G(0) & \text{ if }i=j,\\
      0 & \text{ otherwise.}
  \end{cases}
  \]
For the sake of simplicity, we refer to the previous framework as ``Schied and Zhang market-impact game".
However,
in contrast to \cite{schied2018market}, we assume a permanent market impact as in 
\cite{almgren2001optimal}. So,
 $G(t)\equiv G\in\R_+$ $\forall t$ and the assumptions of strictly 
positive definite (in the sense of Bochner) of $t\mapsto G(|t|)$
no longer holds. In particular, the kernel matrix $\Gamma=G \bm{e}\bm{e}^T \in 
\R^{(N+1)\times (N+1)}$ is singular.
  However, the existence and uniqueness of Nash Equilibrium 
  associated with the two agents ($\bm{\xi}^*$, $\bm{\eta}^*$)
    is guaranteed when 
   $\Gamma_{\theta}:=\Gamma+2\theta I$ is definite positive,   and the matrices $\Gamma_{\theta}\pm\widetilde{\Gamma}$ are invertible ({\color{blue}Nel caso in cui G è costante non ho garanzia che queste matrici siano positive, ma basta averle non-singolari}),
     see proof of Theorem 1 and Lemma 3 and 4 of 
  \cite{schied2018market}.
   Thus, by the matrix determinant lemma\footnote{If $A\in\R^{N\times N}$ is a non singular square matrix and $\bm{u},\bm{v}\in \R^N$, then 
$\det(A+\bm{uv}^T)=(1+\bm{v}^T A^{-1} \bm{u})\det(A)$. 
}, see also Theorem 1 of \cite{ding2007eigenvalues}, the eigenvalues of $\Gamma_{\theta}$
are $
\lambda_1=G \cdot (N+1)+2\theta\text{ and }\lambda_{2:(N+1)}=2\theta,$
so it is definite positive as long as $\theta>0$.
$\Gamma_{\theta}-\widetilde{\Gamma}=\widetilde{\Gamma}^T+2\theta I$ is 
an upper triangular matrix where its diagonal elements are different from zero, i.e., it is 
non singular and finally $\Gamma_{\theta}+\widetilde{\Gamma}  $
is non singular if $\theta>0$, see Appendix 
\ref{app_1}.
Therefore, provided that $\theta>0$, also when $G(t)=G>0$ is constant the Nash equilibrium exists and it is 
given by the previous equations. 

\subsection{Model Setting}

We now specify the two market models we are going to consider.

\subsubsection{The Nash Equilibrium for the Primary Market Model}\label{sec_ne_primary_model}
The previous framework, a Schied and Zhang market-impact game with constant impact function, is employed as
the primary market model.
We remark that the market impact function, which we denote as $G_1\in\R_+$, is constant in time .
Without loss of generality we may fix $G_1= 1$ and
in order to prevent market instability\footnote{The instability appears as a result of oscillating Nash equilibria which in turns affect price dynamics, see \cite{cordoni2020instabilities}. 
However, if $\theta\geq G(0)/4$ these spurious oscillations disappear, see \cite{schied2018market}.} we 
set $\theta\geq G_1/4$, e.g., $\theta=1$.

We consider the interaction between a Directional Seller and
an Arbitrageur, where without loss of generality we may assume that their inventory are given by
$X_{direc}=1$ and $X_{arb}=0$, respectively. 
%arrivato qui 16/12/2020
Then, the Nash equilibrium for the Directional is given by 
the average of the fundamental vectors $\bm{v}$ and $\bm{w}$
Interestingly both the optimal strategies are symmetric in time as described as follows.
In general, the Nash equilibrium depends on the size 
of the inventory of the Directional trader.


\begin{lem}\label{lem_inv_gamma}
Let $\theta>0$, then the inverse of the following matrices
$$(\Gamma_{\theta}-\widetilde{\Gamma}) =
G_1\begin{bmatrix}
\frac{2\theta}{G_1}+\frac{1}{2} & 1 & 1
&\cdots  &1 &1 \\
0&\frac{2\theta}{G_1}+\frac{1}{2} & 1   &\cdots &1 &1\\
0 &\ddots&\ddots &\ddots &\ddots  &\vdots  \\
\vdots &\ddots&\ddots &\ddots &\ddots  &\vdots  \\
\vdots &\ddots&\ddots &\ddots &\frac{2\theta}{G_1}+\frac{1}{2}  & 1  \\
0&\cdots &\cdots&\cdots &0 &\frac{2\theta}{G_1}+\frac{1}{2}  
\\
\end{bmatrix}
$$
$$(\Gamma_{\theta}+\widetilde{\Gamma}) =
G_1\begin{bmatrix}
\frac{2\theta}{G_1}+\frac{3}{2} & 1 & 1
&\cdots  &1 &1 \\
2&\frac{2\theta}{G_1}+\frac{3}{2} & 1   &\cdots &1 &1\\
2 &\ddots&\ddots &\ddots &\ddots  &\vdots  \\
\vdots &\ddots&\ddots &\ddots &\ddots  &\vdots  \\
\vdots &\ddots&\ddots &\ddots &\frac{2\theta}{G_1}+\frac{3}{2}  & 1  \\
2&\cdots &\cdots&\cdots &2 &\frac{2\theta}{G_1}+\frac{3}{2}  
\\
\end{bmatrix}
$$
are given by the matrices,
$$
(\Gamma_{\theta}-\widetilde{\Gamma})^{-1}=\frac{1}{G_1} 
\begin{bmatrix}
\frac{1}{\lambda}&
-\frac{1}{\lambda^2}&
-\frac{\lambda-1}{\lambda^3}&\cdots&
 -\frac{(\lambda-1)^{N-2}}{\lambda^N}&
-\frac{(\lambda-1)^{N-1}}{\lambda^{N+1}} 
  \\
0&   \frac{1}{\lambda}&-\frac{1}{\lambda^2}&\cdots & -\frac{(\lambda-1)^{N-3}}{\lambda^{N-1}}&
  -\frac{(\lambda-1)^{N-2}}{\lambda^{N }} 
  \\
 0& \ddots & \ddots & \ddots &\ddots &\vdots \\
  \vdots& \ddots & \ddots & \ddots &\ddots &\vdots \\
  \vdots& \ddots & \ddots & \ddots &\frac{1}{\lambda} &-\frac{1}{\lambda^2} \\
 0& \cdots & \cdots & \cdots & 0 &\frac{1}{\lambda} 
\\
\end{bmatrix},
$$

$$
(\Gamma_{\theta}+\widetilde{\Gamma})^{-1}=
(\Gamma_{\theta}-\widetilde{\Gamma})^{-T}-G_1\cdot\frac{
(\Gamma_{\theta}-\widetilde{\Gamma})^{-T}\bm{e} \bm{e}^T(\Gamma_{\theta}-\widetilde{\Gamma})^{-T}}
{1+G_1\cdot\bm{e}^T(\Gamma_{\theta}-\widetilde{\Gamma})^{-T}\bm{e}},
$$
 where $\lambda=\frac{2\theta}{G_1}+\frac{1}{2}$.
 \end{lem}
\begin{proof}[Proof of Lemma \ref{lem_inv_gamma}]
The computation of $(\Gamma_{\theta}-\widetilde{\Gamma})^{-1}$ is 
straightforward, see also proof of Proposition 3 of \cite{schied2018market}.
For $(\Gamma_{\theta}+\widetilde{\Gamma})^{-1}$
we may use the Sherman–Morrison formula.
Indeed, $(\Gamma_{\theta}+\widetilde{\Gamma})=
(\Gamma_{\theta}-\widetilde{\Gamma})^T+G_1\bm{e}\bm{e}^T
$, then since $(\Gamma_{\theta}-\widetilde{\Gamma})^T$
is non singular by the Sherman–Morrison formula we have the results,
$(\Gamma_{\theta}+\widetilde{\Gamma})^{-1}=
(\Gamma_{\theta}-\widetilde{\Gamma})^{-T}-G_1\cdot\frac{
(\Gamma_{\theta}-\widetilde{\Gamma})^{-T}\bm{e} \bm{e}^T(\Gamma_{\theta}-\widetilde{\Gamma})^{-T}}
{1+G_1\cdot\bm{e}^T(\Gamma_{\theta}-\widetilde{\Gamma})^{-T}\bm{e}}.$
\end{proof} 

    \begin{pr}\label{direc_solut_symm}
    Let $\theta>0$, then the fundamental solutions, $\bm{v}$ and $\bm{w}$, of a Schied and Zhang market-impact game where the market impact function $G$ is constant, are equal up to a time-symmetry i.e., 
    \begin{equation}
\bm{v}_{k}=\bm{w}_{N+2-k}, \ k=1,2,\cdots,N+1.
\end{equation}
Furthermore, if we denote $(\Gamma_{\theta}+\widetilde{\Gamma})=A$,
  \begin{equation}\label{explicit_fund_solut}
  \bm{v}=
  \frac{
 A^{-T}\bm{e}}
{\bm{e}^TA^{-T}\bm{e}}, \quad
     \bm{w}=
     \frac{
  A^{-1}\bm{e}}
{\bm{e}^TA^{-1}\bm{e}},
\end{equation}
and $v_1=\frac{1}{\lambda \cdot (1-a^{N+1})}$ and 
$v_n=\frac{a^{n-1}}{\lambda \cdot (1-a^{N+1})}$ for $n=2,\ldots,N+1$,
where $\lambda=2\theta/G+\frac{1}{2}$ and $a=1-1/\lambda.$

    \end{pr}
    \begin{proof}[Proof of Proposition \ref{direc_solut_symm}]
    Without loss of generality we may assume that $G=1$. Indeed, let $\bm{\xi}_{1,\cdot}$ and $\bm{\xi}_{2,\cdot}$ be the admissible strategy for $X_1$ and $X_2$ respectively. Then, since $G$ is constant, we may scale the trading strategies by $G$. In particular, we may introduce 
    $\bm{\eta}_{i,\cdot}=G\cdot \bm{\xi}_{i,\cdot}$ for $i=1,2$, i.e.,
    the corresponding admissible strategies for the transformed inventory $Y_i=G\cdot X_i $,  $i=1,2$. Then, the two games are equivalent since,
   $  S_t^{\Xi}= S_t^0 -\sum_{t_k <t} G (\xi_{1,k}+\xi_{2,k})=S_t^0 -\sum_{t_k <t} (\eta_{1,k}+\eta_{2,k}), 
   \ \forall\ t \in \numberset{T}$. 
  If we denote $(\Gamma_{\theta}-\widetilde{\Gamma})=A$,
   then by Lemma \ref{lem_inv_gamma},
   $(\Gamma_{\theta}+\widetilde{\Gamma})^{-1}=A^{-T}-\frac{
A^{-T}\bm{e} \bm{e}^TA^{-T}}
{1+\bm{e}^TA^{-T}\bm{e}}.$
However, 
$$(\Gamma_{\theta}+\widetilde{\Gamma})^{-1}\bm{e}=A^{-T}\bm{e}-A^{-T}\bm{e}\cdot\frac{
 \bm{e}^TA^{-T}\bm{e}}
{1+\bm{e}^TA^{-T}\bm{e}}=A^{-T}\bm{e}\cdot \bigg(1-\frac{
 \bm{e}^TA^{-T}\bm{e}}
{1+\bm{e}^TA^{-T}\bm{e}}\bigg)= \frac{
 A^{-T}\bm{e}}
{1+\bm{e}^TA^{-T}\bm{e}}.$$
   Thus, $\bm{e}^T(\Gamma_{\theta}+\widetilde{\Gamma})^{-1}\bm{e}=\frac{
 \bm{e}^T A^{-T}\bm{e}}
{1+\bm{e}^TA^{-T}\bm{e}}$, so
  \[
  \begin{split}
  \bm{v}&=\frac{1}{\bm{e}^T (\Gamma_{\theta}+\widetilde{\Gamma})^{-1}\bm{e}}(\Gamma_{\theta}+\widetilde{\Gamma})^{-1}\bm{e}=
  \frac{
 A^{-T}\bm{e}}
{\bm{e}^TA^{-T}\bm{e}}
  \\
     \bm{w}&=\frac{1}{\bm{e}^T (\Gamma_{\theta}-\widetilde{\Gamma})^{-1}\bm{e}}(\Gamma_{\theta}-\widetilde{\Gamma})^{-1}\bm{e}=
     \frac{
  A^{-1}\bm{e}}
{\bm{e}^TA^{-1}\bm{e}}.
        \end{split}\]
Moreover, if we denote $A^{-1}\bm{e}=\bm{x}$ and using the explicit formula for $A^{-1}$ we obtain that
$x_{N+1}=\frac{1}{\lambda}$, $x_n=\frac{1}{\lambda}-
\frac{1}{\lambda^2}\sum_{k=0}^{N-n} \left(\frac{\lambda-1}{\lambda}\right)^k=
\frac{1}{\lambda}-
\frac{1}{\lambda}(1-a^{N-n+1})=\frac{a^{N-n+1}}{\lambda}
$, for $n=1,\ldots,N$, where $\lambda=2\theta+\frac{1}{2}$ and $a=\frac{\lambda-1}{\lambda}$. Then, 
$\sum_{n=1}^{N+1}x_n=
\frac{a^N}{\lambda}
\sum_{n=1}^{N+1}a^{-(n-1)}=\frac{a^N}{\lambda}
\sum_{k=0}^{N}a^{-k}=
\frac{a^{N}}{\lambda}\cdot\frac{1-a^{-(N+1)}}{1-a^{-1}}=1-a^{N+1}$, since $1-a=\frac{1}{\lambda}$.
Therefore, $w_{N+1}=\frac{1}{\lambda \cdot (1-a^{N+1})}$ and 
$w_n=\frac{a^{N-n+1}}{\lambda \cdot (1-a^{N+1})}$ for $n=1,2,\ldots,N$. On the other hand, if 
    $A^{-T}\bm{e}=\bm{y}$,
$y_{1}=\frac{1}{\lambda}$, $y_n=\frac{1}{\lambda}-
\frac{1}{\lambda^2}\sum_{k=0}^{n-2} \left(\frac{\lambda-1}{\lambda}\right)^k=
\frac{1}{\lambda}-
\frac{1}{\lambda}(1-a^{n-1})=\frac{a^{n-1}}{\lambda}
$, for $n=2,\ldots,N+1$. Then, 
$\sum_{n=1}^{N+1}y_n=
\frac{1}{\lambda}
\sum_{n=1}^{N+1}a^{n-1}=\frac{1-a^{N+1}}{(1-a)\lambda}=1-a^{N+1}$.
Therefore, $v_1=\frac{1}{\lambda \cdot (1-a^{N+1})}$ and 
$v_n=\frac{a^{n-1}}{\lambda \cdot (1-a^{N+1})}$ for $n=2,\ldots,N+1$.
    \end{proof}

\begin{te}\label{NE_symm}
In a Schied and Zhang market-impact game where the two agents are a Directional and an Arbitrageur,
then the Nash Equilibrium 
is given by the following:
\begin{align}\label{eq_1_S&Z_te}
\bm{\xi}_{direc,\cdot}^*&=\frac{1}{2} X_{direc}( \bm{v}
+\bm{w}),
\\
\label{eq_2_S&Z_te}
\bm{\xi}_{arbi,\cdot}^*&=\frac{1}{2} X_{direc}( \bm{v}
-\bm{w}),
\end{align}
where $\bm{v}$ and $\bm{w}$ are the fundamental solutions and $X_{direc}$ is the inventory of the directional agent.
Moreover, if 
the market impact function is constant and $\theta>0$, the Nash equilibrium is time-symmetric, i.e., 
\begin{align}\label{eq_symm_NE}
{\xi}_{direc,k}^*&={\xi}_{direc,N+2-k}^*, \ k=1,2,\cdots,N+1, \\
{\xi}_{arbi,k}^*&=-{\xi}_{arbi,N+2-k}^*, \ k=1,2,\cdots,N+1. 
\label{eq_symm_NE_2}
\end{align}
\end{te}

\begin{proof}[Proof of Theorem \ref{NE_symm}]
Without loss of generality we may assume that first agent is the Directional, so that $X_1=X_{direc}$ and $X_2=X_{arbi}=0$.
From \cite{schied2018market} the Nash equilibrium is 
provided by Eq. \eqref{eq_1_S&Z}-\eqref{eq_2_S&Z}, and we have Eq. 
\eqref{eq_1_S&Z_te}-\eqref{eq_2_S&Z_te}.
Then, since $\bm{v}$ and $\bm{w}$ are time-symmetric from Lemma \ref{direc_solut_symm} we have 
\[
\begin{split}
{v}_1\pm{w}_1 &=
{w}_{N+1}\pm{v}_{N+1}\\
{v}_k\pm{w}_k &=
{w}_{N+2-k}\pm{v}_{N+2-k},
\end{split}
\]
and it is straightforward to verify Eq. \eqref{eq_symm_NE}-\eqref{eq_symm_NE_2}
\end{proof}
%mettere anche per la matrice gamma_+
In the standard single-agent \cite{almgren2001optimal} framework, 
the optimal 
schedule for the Directional is to trade with a constant rate over the trading periods.
However, 
when in the primary market model 
we specify a constant market impact game, the optimal solution for the Directional provided by the Nash equilibrium has a U-shape, while for the Arbitrageur the optimal schedule 
has a round-trip shape, see Figure \ref{fig_ne_shape},
although it is assumed a permanent impact model as 
\cite{almgren2001optimal}.

 
\begin{co}\label{cor_Ushape}
In a Schied and Zhang market-impact game where the two agents are a Directional, with inventory $X_{direc}>0$, and an Arbitrageur, the market impact $G_1$ is constant
and $\theta>\theta^*=G_1/4$, the Nash equilibrium of the Directional, $\bm{\xi}_{direc,\cdot}^*$, has a U-shape, i.e., it is time-symmetric, positive, strictly decreasing in the first $\lfloor{N/2+1}\rfloor$ components and convex, where $N+1$ is the number of trading time.
\end{co}
\begin{proof}[Proof of Corollary \ref{cor_Ushape}]
WLOG we may assume $G_1=1$.
From Theorem \ref{NE_symm} we have the time-symmetry. 
On the other hand,
from the characterization of the fundamental solution
$\bm{v}$ and $\bm{w}$, see Proposition 
\ref{direc_solut_symm}, 
$\bm{\xi}_{direc,k}^*=\frac{X_{direc}}{2}\cdot \frac{a^{k-1}+a^{N-k+1}}{\lambda (1-a^{N+1})}$, 
where $\lambda=2\theta+1/2$ and $a=1-1/\lambda$.
Since $\theta >1/4$, then $\lambda >1$ and $a\in (0,1)$ so each component of the Nash equilibrium is positive. 
Let us denote with $\widetilde{\xi}_k$ the components of 
$\widetilde{\bm{\xi}}=\frac{2 \bm{\xi}_{direc,k}^*}{X_{direc}} $.
Let $\Delta_k=\widetilde{\xi}_{k+1}-\widetilde{\xi}_k$
be the first difference for $k=1,2,\ldots,N$. Then, since 
$\lambda (1-a^{N+1})>0$,
$\Delta_k=\frac{(a-1)(a^{k-1}-a^{N-k})}{\lambda (1-a^{N+1})}=
\frac{(a-1) a^{-k} (a^{2k-1}-a^N)}{\lambda (1-a^{N+1})}<0$
for $k<\lfloor{N/2+1}\rfloor$. For the convexity we consider 
the first difference of $\Delta_k$, i.e., $\Delta_k-\Delta_{k-1}$
for $k=2,3,\ldots,N$. However,
$\Delta_k-\Delta_{k-1}=\frac{(a-1)(a^{k-1}-a^{N-k})-(a-1)(a^{k-2}-a^{N-k+1})}{\lambda (1-a^{N+1})}=\frac{(a-1)(a^{k-1}-a^{N-k}-a^{k-2}+a^{N-k+1})}{\lambda (1-a^{N+1})}=\frac{(a-1)(a-1)(a^{k-2}+a^{N-k})}{\lambda (1-a^{N+1})}>0$ and we conclude.
\end{proof}
 



      \begin{figure}[t]
\centering
{\includegraphics[width=1\textwidth]{plot_new/AC_fund_arbit.eps}}
\caption{ Nash equilibrium $\bm{\xi}_{direc}^*$ of the Directional
and $\bm{\xi}_{arbi}^*$ of the Arbitrageur trading only one asset. The trading time grid is equidistant with 26 points and 
$\theta=1$. The market impact is constant $G_1=1.$} 
\label{fig_ne_shape}
\end{figure}

\subsubsection{The Nash Equilibrium for the Secondary Market Model}

In the secondary market model we consider only the price impact of the Directional without any type of interactions with other agents.
To avoid confusion with the primary market model 
strategies
and for the sake of simplicity we denote with $\bm{\eta}$ the admissible strategy 
for the secondary market model.
As also highlighted by \cite{schied2018market},
the optimal solution for a Directional with inventory $X_{direc}$ is obtained by 
\[
\bm{\eta}_{direc}^{*}=\frac{X_{direc}}{\bm{e}^T\Gamma_{\theta}^{-1} \bm{e} }
\Gamma_{\theta}^{-1} \bm{e},
\]
where $\Gamma_{\theta}$ is the corresponding decay matrix
for the market impact function $G_{2}(t)$ of the secondary market model.
Since $\Gamma_{\theta}$ is symmetric then it is trivial that 
$\bm{\eta}_{direc}^{*}$ is also time symmetric as $\bm{\xi}^*_{direc}$.
Moreover, it is straightforward that if we assume 
a constant market impact function $G_2$ the solution of $\bm{\eta}^*_{direc}$ is constant among time, i.e., the classical \cite{almgren2001optimal} solution. 
In the general case, where $G_2(t)$ is a strictly positive decay kernel, the secondary market impact model is essentially the standard TIM with no competitors.
Then, as it is well known, 
 the optimal execution is characterized by U-shape, e.g., see Figure \ref{fig_ne_shape_TIM}. 
 
 

   \begin{figure}[t]
\centering
{\includegraphics[width=0.75\textwidth]{plot_new/xi_tim.eps}}
\caption{Nash equilibrium $\bm{\eta}_{direc}^*$ of the Directional in a TIM model when there is no interactions. 
The trading time grid is equidistant with 26 points and 
$\theta=1$. The market impact function is an exponential decay kernel $G_2(t)=\exp(-t).$} 
\label{fig_ne_shape_TIM}
\end{figure}


\section{The Intrinsic Transient Impact Function}

We now address our main question.
We observe that,
by the results of the previous Section, when in the 
primary market model we set a constant market impact function $G_1\in \R_+$ the optimal solution
of the directional provided by the Nash equilibrium $\bm{\xi}^*_{direc}$ of the related market impact game
has a U-shape. The same U-shape is also exhibited 
by the optimal schedule provided by the secondary market model, 
when a suitable transient impact function is selected, i.e.,
the U-shape of $\bm{\xi}^*_{direc}$ is equivalent to optimal schedules obtained by single-agent Transient Impact Models. 
Therefore, given the optimal solution $\bm{\xi}_{direc}^*$
it is possible to fit an appropriate propagator function 
so that $\bm{\xi}^*_{direc}=\bm{\eta}^*_{direc}$.
We denote this transient impact function as $G_{intr}(t)$,
which we name \emph{intrinsic transient impact/decay kernel function}.
The market impact is intrinsically transient in the 
primary market model, where the market impact is extrinsically constant. 

To avoid confusion we emphasize the previous definition.
\begin{de}[Intrinsic transient impact function]\label{def_intrinsic_decay_kernel}
The transient impact function $G_{intr}(t)$ such that 
the optimal schedule obtained by a single TIM, $\bm{\eta}^*_{direc}$, is equal to the Nash equilibrium of the Directional in the primary market model, $\bm{\xi}^*_{direc}$, is called \emph{intrinsic transient impact function}.
\end{de}

In particular, it is
the interaction between agents in the market impact game,
with a permanent impact, which generates and characterizes
the intrinsic transient impact. 
In order to make extrinsic\footnote{In the sense that the price impact is described explicitly by $G_{intr}(t)$.} $G_{intr}(t)$ we have to consider 
a model where the is no interaction, 
i.e., the secondary market model.
In other words, in the secondary market model $G_{intr}(t)$ describes the price impact in such a way the interaction
with the Arbitrageur is also considered, i.e., it is intrinsically considered in the propagator function.
So, this suggests that the general transient impact/propagator function is 
an intrinsic effect
produced by
the results of agents interactions. This is in agreement with the results of \cite{vodret2020stationary}.


We remark that the optimal schedule provided by TIM with the intrinsic transient impact function of the secondary market model, it is also optimal for the primary market model.
So, using the intrinsic market impact function we are able to find a solution for the classical TIM which takes into account also the possibility of interaction with an other agent, the arbitrageur.

Now, we address the following question. Given the 
solution obtained by a market impact game, how is it possible 
to derive the corresponding intrinsic decay kernel to be associated to the single-agent TIM?
Moreover, is the intrinsic transient impact function unique?


\subsection{Is it possible to estimate the kernel from the optimal execution?}


%  "Per questa scelta di theta la soluzione esiste anche in tempo continuo"
Without loss of generality we assume $X_{direc}=1$.
Given $\bm{\xi}_{direc}^{*}\in \R^{N+1}$ we ask whether the equation 
\begin{equation}\label{eq_probl_solver}
  \bm{\xi}_{direc}^{*}=\frac{\Gamma_{\theta}^{-1} \bm{e}}{\bm{e}^T\Gamma_{\theta}^{-1} \bm{e} }
\end{equation}
has solution and 
if it is unique. 
Since $\theta>0$ is given, the unknown is the symmetric Toeplitz matrix
$\Gamma$ such that $\Gamma_{\theta}=\Gamma+2\theta I$, which depends on $N+1$ parameters,
thus in principle there are $N+1$ equations in $N+1$ unknowns. However it is clear that if $\Gamma$ is a solution,
then any $\Gamma+K\bm{e} \bm{e}^T$ ($K\in \R$) is a solution, as observed in the following remark. 

 
\begin{os}\label{up_constant}
Using Sherman–Morrison formula, it is straightforward that
$ \frac{(\Gamma_{\theta}+K e e^T)^{-1}e}{e^T(\Gamma_{\theta}+K e e^T)^{-1}e} = \frac{\Gamma_{\theta}^{-1}e}{e^T\Gamma_{\theta}^{-1}e}$, for each $K \in \R$. 
So $G(t)$ and $G(t)+K$, where $K\in \R$,
generate the same optimal execution of a TIM, then the decay kernel is identifiable up to a constant.
\end{os}
 

Moreover,
$\Gamma_{\theta}$ is identified up to a multiplicative constant, i.e., if $\Gamma_{\theta}$ satisfies \eqref{eq_probl_solver}
then any $\alpha \Gamma_{\theta}$ where $\alpha\neq0$ is a solution.
Therefore, we may set $G(0)$ such that the elements of the main diagonal of $\Gamma_{\theta}$, which are $G(0)+2\theta$, are equal to $1$.
 However,
 even if we select a particular class of decay kernel
 we show that in general the identification of $G_{intr}(t)$
is not related only to a constant and multiplicative scaling.


To solve the problem \eqref{eq_probl_solver}, let us set
$$
\Pi^{-1}=\frac{\Gamma_{\theta}^{-1}}{\bm{e}^T\Gamma_{\theta}^{-1} \bm{e} }
$$
hence $$
\Pi=(\bm{e}^T\Gamma_{\theta}^{-1} \bm{e} )\Gamma_{\theta}$$
and we may rewrite Equation \eqref{eq_probl_solver} as
\begin{equation}\label{eq_probl_solver2}
\Pi \bm{\xi}_{direc}^{*} =\bm{e}  
\end{equation}
where the unknowns are the $N+1$ different entries of 
$\Pi=\mbox{Toeplitz}(g_0,g_1,\ldots,g_{N})=\mbox{Toeplitz}(\bm{g})$.
Moreover $\Pi$ is symmetric and satisfies $\bm{e}^T \Pi^{-1} \bm{e}=1$.
 Thus, we recast Equation \eqref{eq_probl_solver2}
 into a linear system in the unknowns $\bm{g}$. 
 Let us consider as an example the case of $N+1=4$.
 The original system is formulated as 
 $$
 \begin{bmatrix}
 g_0 & g_1 & g_2 & g_3\\
  g_1 & g_0 & g_1 & g_2\\
   g_2 & g_1 & g_0 & g_1\\
    g_3 & g_2 & g_1 & g_0\\
 \end{bmatrix}
 \begin{bmatrix}
 \xi_1 \\
 \xi_2 \\
   \xi_3 \\
    \xi_4 \\
 \end{bmatrix}=\begin{bmatrix}
 1 \\ 1\\ 1\\1
 \end{bmatrix},
 $$
 where we omit upper $*$ for the sake of simplicity,
 which can be rewritten as
  $$
 \begin{bmatrix}
 \xi_1 & \xi_2 & \xi_3 & \xi_4\\
  \xi_2 & \xi_1+\xi_3 & \xi_4 & 0\\
  \xi_3 & \xi_2+\xi_4 & \xi_1 & 0\\
 \xi_4 & \xi_3 & \xi_2 & \xi_1\\
 \end{bmatrix}
 \begin{bmatrix}
g_0 \\
 g_1 \\
   g_2 \\
    g_3 \\
 \end{bmatrix}=\begin{bmatrix}
 1 \\ 1\\ 1\\1
 \end{bmatrix},
 $$
 i.e., as 
 \begin{equation}\label{eq_with_H}
     H\bm{g}=\bm{e}
 \end{equation}
 from which we may recover $\bm{g}=H^{-1} \bm{e}$. 
 Then, since $\bm{\xi}^*_{direc}$ has a U-shape, in particular it is time-symmetric, Equation \ref{eq_probl_solver2} has in general 
 infinite solutions. This means that there intrinsic transient 
 impact function can not be identified without imposing some restrictions.
 Before
 showing the main results we provide two examples.
 \begin{es}
 If for some reasons $\xi^*_{direc}$ is not time-symmetric (for example it is the result of the Nash equilibrium of a
Directional against $M > 1$ Arbitrageurs, see below) and there are no other symmetries, the matrix $H$ is
full rank and invertible. The unique solution is
 the constant vector $\bm{g}=\frac{\bm{e}}{\bm{e}^T \bm{\xi}^*_{direc}}$, which provides however a singular matrix $\Pi$.
 Therefore, as we expect, when $\xi^*_{direc}$ is not time-symmetric 
 there is no $\Gamma$ which satisfies Equation \eqref{eq_probl_solver}.
 \end{es}
 
 \begin{es}
 Let us consider the case when $N+1=4$ and let us 
 suppose $\xi^*_{direc}$ be a U-shaped.
 As a consequence the matrix $H$ is not full rank.
We recover $\xi^*_{direc}$ by the optimal execution of a TIM where
 $\Gamma_{\theta}= \mbox{Toeplitz}(1, 0.6, 0.5, 0.2)$, 
 thus $\bm{\xi}^*_{direc} = 12^{-1}(5, 1, 1, 5)$. The rank of the matrix $H$ is 2, so the space of the solutions is infinite and it has dimension $2$ and can be 
 parametrized as 
 $\bm{g}=\left(\frac{60}{29}-\frac{\alpha}{29}-\frac{30}{29}\beta,
 \frac{48}{29}-\frac{24}{29}\alpha+\frac{5}{29}\beta,\alpha,\beta\right)$.
 Choosing $\alpha=\beta=0$ one gets $\Pi=\mbox{Toeplitz}(60/29,48/29,0,0)$, which is clearly not proportional to the ``original" $\Gamma_{\theta}$, which can be recovered
 with 
 $\alpha=0.8450704$, $\beta = 0.3380282$, getting $\Pi=1.6901408\Gamma_{\theta}$.
 \end{es}

 \begin{te}[Identification Problem of the Intrinsic Transient Impact Function]\label{id_intrinsic_decay}
 Let us suppose that $\bm{\xi}^*_{direc}\in \R^{N+1}$ has a U-shape, 
 then the system 
 \begin{equation}\label{eq_probl_solver2}
\Pi \bm{\xi}_{direc}^{*} =\bm{e} \Longleftrightarrow
H\bm{g}=\bm{e}
\end{equation}
where $\Pi=\mbox{Toeplitz}(\bm{g})$ is symmetric
and $\bm{g}\in \R^{N+1}$ has strictly decreasing components {\color{red} non serve ipotesi di Toep}, has infinite solutions, where the rank of $H$ is equal to $(N+1)/2$ if $N+1$ is even and $N/2+1$ if $N+1$ is odd, respectively.
 \end{te}
 \begin{proof}[Proof of Theorem \ref{id_intrinsic_decay}]
  Let us first consider the case when $N+1$ is even.
  From the lhs, since $\Pi$ is symmetric and $\bm{\xi}^*_{direc}$
  is time symmetric the first $(N+1)/2$ equations are equal to the last $(N+1)/2$, where the first is equal to the $N+1$-th, 
  the second is equal to the $N$-th and so on.
  This, means that $\mbox{rk}(H)\leq (N+1)/2$. However, since $\bm{\xi}_{direc}^*$ has a U-shape {\color{blue}(anche il fatto che è positivo)}, in particular it is not constant but strictly decreasing, and $\bm{g}$ {\color{blue}(e le component di g hanno lo stesso segno)} is strictly decreasing, then the first $(N+1)/2$ equations are different from each other, 
  since for each equation there are mixed products which are not contained in the remaining equations. Thus, $\mbox{rk}(H)=(N+1)/2$.
  The case of $N+1$ odd is straightforward, since using the same reasoning as of the even case, we obtain that the first $N/2$ equations are equal to the last $N/2$ where
  in addition we have another equation at the $N/2+1$ coordinate.
  So, $\mbox{rk}(H)=N/2+1.$
 \end{proof}
 In other words, in general, there are $(N+1)/2$ and $N/2$ solutions
 as much possibles intrinsic transient impact functions, when $N+1$ is even and odd, respectively. 
 

\subsubsection{The Intrinsic Linear Transient Impact Function}
\label{sec_linear_TIM}
We now investigate the previous problem when the intrinsic 
decay kernel is assumed to be linear.
We assume that the time grid is equidistant 
$\T_N=\{\frac{kT}{N}|k=0,1,\ldots,N\}$, where $T=1$ and $N\in \N$.
If $G_{intr}(t)=c+m t$, where $m<0$ and, since the
kernel is identified up to a constant term, we impose 
without loss of generality that $c$
 is such that $G_{intr}(T)=0$. The previous matrix $\Pi$
 is proportional up to a constant to the decay kernel matrix $\Gamma_{\theta}$, so we search for a 
 $\Pi=\mbox{Toeplitz}(g_0,g_1,\ldots,g_N)$, where 
 $g_k=2\theta\delta_{k,0}+\alpha+\beta\frac{k}{N}$, for $k=0,1,\ldots,N$ where $\delta_{k,0}$ is $1$ for $k=0$ and 0 otherwise.
 Then, if $X_{direc}$ is the inventory of the Directional, since $\Pi \bm{\xi}_{direc}^*=1$ we may recover\footnote{For the sake of simplicity we remove the upper $*$ and $fund$ from the component of $\xi^*_{direc}$.} the first $\lfloor{N/2+1}\rfloor$:
 \begin{enumerate}[align=left]
     \item[(Eq. 1)] $\alpha X_{direc}+2\theta\xi_1+\frac{\beta}{N} \sum_{i=2}^{N+1}(i-1) \xi_i=1 $;
     \item[(Eq. 2)]  $\alpha X_{direc}+2\theta\xi_2+\frac{\beta}{N}  \left(\xi_1+\sum_{i=3}^{N+1}(i-2) \xi_i\right)=1 $; 
     \item[(Eq. $k$)]  $\alpha X_{direc}+2\theta\xi_3+\frac{\beta}{N} \left((k-1)\xi_1+(k-2)\xi_2+\cdots+2\xi_{k-2}+\xi_{k-1}+
     \sum_{i=k+1}^{N+1}(i-k) \xi_i\right)=1 $, where $k\leq\lfloor{N/2+1}\rfloor$. 
 \end{enumerate}
 {\color{blue} From Corollary \ref{cor_Ushape} if $\theta>\theta^*=G_1/4$, the components of $\bm{\xi}$ 
 are all positive.}
 Thus, subtracting each equation from the previous one we obtain that
 \begin{enumerate}[align=left]
     \item[(Eq. 1) $-$ (Eq. 2)] $2\theta (\xi_1-\xi_2)
     +\frac{\beta}{N} \left( 
     \sum_{i=2}^{N+1} \xi_i-\xi_1
     \right)=0
     $;
     \item[(Eq. $k-1$) $-$ (Eq. $k$)]    $2\theta (\xi_{k-1}-\xi_k)
     +\frac{\beta}{N} \left( 
     \sum_{i=k}^{N+1} \xi_i-     \sum_{i=1}^{k-1} \xi_i
     \right)=0$, where $k\leq\lfloor{N/2+1}\rfloor$.  
 \end{enumerate}
 Therefore,
 since $X_{direc}=\sum_{i=1}^{N+1}\xi_i$,
 we may compute $\beta$ using the previous equation (Eq. 1) $-$ (Eq. 2),
 \[
 \beta=\frac{-2\theta N \cdot (\xi_1-\xi_2)}{X_{direc}-2\xi_1},
 \]
 but from (Eq. $k-1$) $-$ (Eq. $k$)
 \[
 \beta=\frac{-2\theta N \cdot (\xi_{k-1}-\xi_k)}{X_{direc}-2\sum_{i=1}^{k-1}\xi_i},
 \quad k\leq\lfloor{N/2+1}\rfloor.
 \]
 Therefore, it must hold for  $k\leq\lfloor{N/2+1}\rfloor$
 \begin{equation}\label{cond_linear_decay_first}
     \frac{-2\theta N \cdot (\xi_1-\xi_2)}{X_{direc}-2\xi_1}=
     \frac{-2\theta N \cdot (\xi_2-\xi_3)}{X_{direc}-2\xi_1-2\xi_2}=
     \cdots=
     \frac{-2\theta N \cdot (\xi_{k-1}-\xi_k)}{X_{direc}-2\sum_{i=1}^{k-1}\xi_i},
 \end{equation}
 which, since $\theta \neq 0$,  is equivalent to
  \begin{equation}\label{cond_linear_decay}
     \frac{ (\xi_1-\xi_2)}{X_{direc}-2\xi_1}=
     \frac{(\xi_2-\xi_3)}{X_{direc}-2\xi_1-2\xi_2}=
     \cdots=
     \frac{ (\xi_{k-1}-\xi_k)}{X_{direc}-2\sum_{i=1}^{k-1}\xi_i},\
     k\leq\lfloor{N/2+1}\rfloor
     .
 \end{equation}
 {\color{blue}
 \begin{os}\label{os_two_theta}
 We observe that if $\theta=0$, then the relations \eqref{cond_linear_decay_first}
 are satisfied. 
 However, the Nash Equilibrium of the primary market model exists and it has no oscillations when $\theta\geq\theta^*>0$.
 Therefore, we may set two different $\theta$ one for the first market model, $\theta_1$, such that the Nash equilibrium is well defined and one for the secondary market model $\theta_2$ where we set $\theta_2=0$. We discuss this particular case in Section \ref{incor_theta_in_G}.
 \end{os}
 }
 Then, we have proven the following result.
 \begin{te}[Linear Intrinsic Transient Impact Function]
 \label{te_linear_beta_results}
 Let  $\T_N=\{\frac{kT}{N}|N\in \N, \ k=0,1,\ldots,N\}$, 
 be an equidistant time grid and {\color{blue}$\theta>\theta^*=G_1/4$}.
 $\Pi=\mbox{Toeplitz}(\bm{g})$, where 
 $g_k=2\theta\delta_{k,0}+\alpha+\beta\frac{k}{N}$, $k=0,1,\ldots,N$ is a solution for \eqref{eq_probl_solver2} if 
 and only if
  the components of $\bm{\xi}^*_{direc}$  
 satisfy the relation \eqref{cond_linear_decay}.
 Moreover, 
 $\beta= \frac{-2\theta N \cdot (\xi_{1}-\xi_2)}{X_{direc}-2\xi_1}$.
 \end{te}
 
 We observe that the components of $\xi^*_{direc}$  
 satisfy the relation \eqref{cond_linear_decay} if and only if
 $\frac{ (\xi_{k-1}-\xi_k)}{X_{direc}-2\sum_{i=1}^{k-1}\xi_i}$ is independent from $k$.
 Furthermore, we show that the Nash equilibrium 
 of the Directional $\bm{\xi}^*_{direc}$ provided by the 
 primary market model satisfies the previous conditions.
 
 \begin{pr}\label{pr_linear_xi}
 The components of $\bm{\xi}^*_{direc}$ satisfy 
 \eqref{cond_linear_decay}.
 \end{pr}
 \begin{proof}[Proof of Proposition \ref{pr_linear_xi}]
 WLOG we may assume the impact function of the primary market model $G_1=1$.
 From the characterization of the fundamental solutions 
 $\bm{v}$ and $\bm{w}$, see Proposition \ref{direc_solut_symm},
 ${\xi}_{direc,k}^*=\frac{X_{direc}}{2}\cdot \frac{a^{k-1}+a^{N-k+1}}{\lambda (1-a^{N+1})}$, 
 where $\lambda=2\theta+\frac{1}{2}$ and $a=1-1/\lambda$.
 So, let $\xi_k$ be the components of $\bm{\xi}_{direc}^*$, then, 
 for $k\leq\lfloor{N/2+1}\rfloor$,
 \[
 \frac{(\xi_{k-1}-\xi_k)}{X_{direc}-2\sum_{i=1}^{k-1}\xi_i}=
\frac{a^{k-2}+a^{N-k+2}-a^{k-1}-a^{N-k+1} }{2\lambda (1-a^{N+1})}\cdot\frac{1}{1-\sum_{i=1}^{k-1} \frac{a^{i-1}+a^{N-i+1}}{\lambda (1-a^{N+1})}   }=
 \]
 \[
 =\frac{a^{k-2}+a^{N-k+2}-a^{k-1}-a^{N-k+1} }{2\lambda (1-a^{N+1})}\cdot\frac{\lambda (1-a^{N+1})}{\lambda (1-a^{N+1})-\sum_{i=1}^{k-1} (a^{i-1}+a^{N-i+1})   }=
 \]
 \[
 =\frac{1}{2}\cdot \frac{a^{k-2}+a^{N-k+2}-a^{k-1}-a^{N-k+1} }{\lambda (1-a^{N+1})-\sum_{i=1}^{k-1} (a^{i-1}+a^{N-i+1})   }.
 \]
 Since $\sum_{i=1}^{k-1}a^{i-1}=(1-a^{k-1})/(1-a)$ and 
 $a^{N+1}\cdot\sum_{i=1}^{k-1} a^{-i}=(a^{N-k+2}-a^{N+1})/(1-a)$,
 and $\lambda(1-a)=1$
  \[
  \begin{split}
 &\frac{1}{2}\cdot \frac{a^{k-2}+a^{N-k+2}-a^{k-1}-a^{N-k+1} }{\lambda (1-a^{N+1})-\sum_{i=1}^{k-1} (a^{i-1}+a^{N-i+1})   }\\ =&\frac{1-a}{2}\cdot \frac{a^{k-2}+a^{N-k+2}-a^{k-1}-a^{N-k+1} }{\lambda(1-a) (1-a^{N+1})-(1-a^{k-1}+a^{N-k+2}-a^{N+1})  }
 \\
 =&
 \frac{1-a}{2}\cdot \frac{a^{k-2}+a^{N-k+2}-a^{k-1}-a^{N-k+1} }{a^{k-1}-a^{N-k+2} }=
 \frac{1-a}{2}\cdot \frac{a^{k-2}(1-a)-a^{N-k+1}(1-a) }{a^{k-1}-a^{N-k+2} }\\
 =&\frac{(1-a)^2}{2}\cdot \frac{a^{k-2}-a^{N-k+1}}{a^{k-1}-a^{N-k+2} } 
 =\frac{a(1-a)^2}{2a}\cdot \frac{a^{k-2}-a^{N-k+1}}{a^{k-1}-a^{N-k+2} } 
 =\frac{(1-a)^2}{2a}\cdot \frac{a^{k-1}-a^{N-k+2}}{a^{k-1}-a^{N-k+2} } \\
 =&\frac{(1-a)^2}{2a}.
\end{split}
 \]
 Therefore, $\frac{(\xi_{k-1}-\xi_k)}{X_{direc}-2\sum_{i=1}^{k-1}\xi_i}=\frac{(1-a)^2}{2a}$ and so it is independent for each $k\leq\lfloor{N/2+1}\rfloor$ and we conclude.
 \end{proof}
 
 
 This implies that there exists an intrinsic linear decay kernel $G_{intr}(t)$ which satisfies \eqref{eq_probl_solver}.
 The slope is provided by 
 $-\theta N \frac{(1-a)^2}{a}=
 -\frac{4\theta N G_1^2}{16\theta^2-G_1^2}
 $, since $a=1-1/\lambda$,
 $\lambda=2\theta/G_1+\frac{1}{2}$ and $G_1$ is the permanent market impact function of the primary market model.
 {\color{blue}
 Since $\theta > G_1/4$ then the slope is always negative, i.e., the linear intrinsic market impact 
 functions are effectively decay kernels.
 We also observe that this slope is an increasing function of $G_1$ and it decreases with $\theta$. We further investigate this latter relation 
 in Section \ref{transaction_cost_effect}
 In particular,
 this means that linear solutions of $\eqref{eq_probl_solver}$ are contained in a one dimensional affine space, so 
 if we impose that $G_{intr}(T)=0$, then we may identify
 the unique intrinsic linear transient impact function.
  }





 

\subsection{Fitted Intrinsic Transient Impact Functions}\label{sec_numerical_fit}
{\color{blue}
Even if in principle there exist infinite solutions of \eqref{eq_probl_solver}, we try to fit an intrinsic decay kernel numerically given the Nash equilibrium $\bm{\xi}_{direc}^*$
of the primary market model.
We conduct some numerical experiments to analyze if the linear solution have a peculiar role and to investigate if there are any other nonlinear candidates as intrinsic decay kernels.
We first try to fit a decay kernel in a non parametric way. 
 Then, we specify some family of decay kernel and we perform a 
parametric fit. 

\subsubsection{Non Parametric Fitting}\label{sec_non_param_fitting}
We now try to fit $G_{intr}(t)$ without imposing 
any type of parametric constraints. We only impose that the decay kernel must be convex and decreasing. Since the kernel is identified up to a constant, we fix $G_{intr}(T)=0$.
We consider a primary market model with an equidistant 
time grid $\T_N=\{\frac{kT}{N}| k=0,1,\ldots,N\}$, where
$T=1$, $N=25$, $G_1=1$, $\theta=1$.
The inventory of the two risk-neutral agents are equal to $1$ and $0$, respectively, as usual.
As observed by Remark \ref{up_constant}, the kernel is
identified up to a constant.
Thus, we impose 
for each fitted kernel that $G(T)=0$.
From Theorem \ref{te_linear_beta_results} we may 
identify the slope $\beta$ of the linear intrinsic decay kernel which is given by $\beta= -\frac{4\theta N G_1^2}{16\theta^2-G_1^2}=-6.6667$.
We start by selecting $100$ different starting points 
using 50 exponential and 50 power law decay kernels.
Figure \ref{fig_non_par_fitting1} reports the starting points from the exponential and power law decay kernels, panels (a) and (b), respectively, and the fitted 
intrinsic decay kernel.
The average error between $\bm{\xi}_{direc}^*$ 
and 
the fitted $\bm{\eta}_{direc}^*$ is $2.0938 e-05$.
Even if 
some fitted intrinsic decay kernel seems to be
nonlinear, we observe that all the fitted kernel seems to be close to the linear intrinsic decay kernel 
$-6.6667\cdot t+6.6667$.
We repeat the previous analysis by choosing different starting points. As before,
Figure \ref{fig_non_par_fitting2} reports the starting points from the exponential and power law decay kernels, panels (a) and (b), respectively, and the fitted 
intrinsic decay kernel.
In this case the average error between $\bm{\xi}_{direc}^*$ 
and 
the fitted $\bm{\eta}_{direc}^*$ is $1.6226e-07$.
Moreover, all the fitted intrinsic decay kernel coincides, for almost all points, with the linear 
linear intrinsic decay kernel. 
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.4]{plot_new/fitted_decay_kernel_nonparam1.eps}
    \caption{First non parametric fitting. 100 starting points from the exponential and power law decay kernels, panels (a) and (b), respectively, and the fitted 
intrinsic decay kernel, right panel. The primary market model has an equidistant time grid $T=1$, $N=25$, $G_1=1$, $\theta=1$.
The inventory of the two risk-neutral agents are equal to $1$ and $0$, respectively.}
    \label{fig_non_par_fitting1}
\end{figure}
\begin{figure}[!t]
\centering
    \includegraphics[scale=0.4]{plot_new/fitted_decay_kernel_nonparam2.eps}
    \caption{Second non parametric fitting. 100 starting points from the exponential and power law decay kernels, panels (a) and (b), respectively, and the fitted 
intrinsic decay kernel, right panel. The primary market model has an equidistant time grid $T=1$, $N=25$, $G_1=1$, $\theta=1$.
The inventory of the two risk-neutral agents are equal to $1$ and $0$, respectively.}
    \label{fig_non_par_fitting2}
\end{figure}

From this analysis the linear intrinsic decay kernel appears to be a privilege candidate as intrinsic decay kernel. 
Therefore, we did not find any particular evidence of other possible families of 
$G_{intr}(t)$. Thus, we further investigate if the linear solution is the unique family of $G_{intr}(t)$ using parametric fitting.


\subsubsection{Parametric Fitting}

We select three family for the intrinsic decay kernel function:
\begin{itemize}
\item polynomial, $G_{intr}^{pol}(t)= \alpha_2 t^2+\alpha_1 t+\alpha_0$;
\item exponential $G_{intr}^{exp}(t)=\lambda e^{-\rho t}+\gamma$;
\item power law $G_{intr}^{pow}(t)=\frac{B}{(1+t)^{1-p}}+C$.
\end{itemize}

Then, we can easily fit the parameters from the
directional seller solution of a market impact game in the primary market model.  
% We assume momentarily that $\theta$ is the same for 
% both the market impact game and the single-agent TIM for the secondary market model. 
% In the next section we discuss how to relax this assumption.
We select the same setting as above, an equidistant time grid where $T=1$, $N=25$, $G=1$, $\theta=1$ where we impose a constraint on the 
intercept terms $\alpha_0$, $\gamma$, $C$ such that $G_{intr}(T)=0$.


Table \ref{tab_fitted_kernel} exhibits the 
fitted parameters for the various decay kernel.
By comparing the residual sum of squares, the best fit is provided by the polynomial  family. The power law fitting provides non significant estimate of the coefficient $B$. 
Moreover, the quality of the fit is very poor compared to the first two families.
We observe from Figure 
\ref{fig_decay_kernel} and \ref{fig_ne_ac_tim} that the most appropriate 
family is the linear one followed by the exponential decay, which is however
also very close to be linear.
In particular, it is quite evident that the solution provided 
by the power law family does not produce a good fit.


\begin{table}[t]
\centering
\caption{Fitted parameters for the three different intrinsic decay kernel families.
For each parameters it is reported the estimate, standard error and confidence interval at 95\%. Res.norm is 
the value of the squared 2-norm of the residual. The intercept term for each fitted kernel is selected in such a way that $G_{intr}(T)=0$}
\label{tab_fitted_kernel}
\begin{tabular}{lllll}
\toprule
    & Estimate            & SE       & CI 95\%    &            \\
    \midrule
    Polynomial\\
 $\alpha_2$ & -0.3671e-05 &   0.0867e-05 &  -0.5460e-05 &   -0.1881e-05  \\
 $\alpha_1$ & -6.6667  &  2.2622e-06  & -6.6667 &  -6.6667\\
Res.norm & 1.0641e-14\\
\midrule
  Exponential\\
 
$\lambda$ & 193.7472  & 38.5179 & 114.2502 & 273.2442\\
 $\rho$   & 0.0357   & 0.0074   & 0.0204  &  0.0509\\
 
Res.norm & 8.3847e-06 \\
\midrule 
Power-law\\
$p$ & 0.9954  &  0.2321  &  0.5163  &  1.4745  \\
   $B$ & 0.0288e05 &    1.4410e05 &  -2.9453e05 &   3.0029e05    \\
     Res.norm & 0.0026       \\
    \bottomrule
\end{tabular}
\end{table}


     \begin{figure}[t]
\centering
{\includegraphics[width=0.85\textwidth]{plot_new/fitted_kernel_param.eps}}
\caption{ The fitted decay kernel among the three selected 
family.} 
\label{fig_decay_kernel}
\end{figure}

     \begin{figure}[t]
\centering
{\includegraphics[width=0.85\textwidth]{plot_new/TIM_with_fitted_kernel_on_AC.eps}}
\caption{Nash equilibrium $\bm{\xi}_{direc}^*$ of the Directional
obtained by a market impact game of the primary market model with permanent impact (green), 
and 
Nash equilibrium $\bm{\eta}_{direc}^*$ for the secondary market model with the fitted polynomial (cyan), exponential (blue) and power intrinsic decay kernel (red).
} 
\label{fig_ne_ac_tim}
\end{figure}

Over all, even if we specify specify a family to the 
intrinsic decay kernel, the linear solution seems to be the unique solution which provides an appropriate fit. We may 
conjecture that the unique intrinsic decay kernel is actually the linear one discussed in Section \ref{sec_linear_TIM}.
}
\section{Transaction Cost Levels and the Intrinsic Decay Kernel}

We examine the relations of the transaction cost levels $\theta$ of the two market models and the intrinsic transient impact function.
We first show how we may incorporate the $\theta$ of the primary market model in the intrinsic decay kernel, so that we may choose zero as the transaction cost level of the secondary market model.
In particular, we generalize the above setting allowing the two market models have different $\theta$. 
Finally, we analyze the sensitivity of the intrinsic decay kernel to the increasing  of transaction costs.

\subsection{Is it possible to incorporate transaction costs in the decay kernel?}\label{incor_theta_in_G}

We now investigate the case when 
the transaction costs of the primary, $\theta_1$, and the secondary, $\theta_2$, market models are different.
In particular, while $\theta_1\geq G_1/4$, we set $\theta_2=0$ for the secondary market model, so that
$\bm{\eta}_{direc}^*$ is characterized by the vector $\Gamma^{-1} \bm{e}$. 
{\color{blue} 
Although
we may imagine that
when $\theta_2=0$ we are looking for
a transient impact function, $G_{intr}(t)$, such that it incorporates the interaction between the two agents together with the 
transaction costs of the primary market model, the economic interpretation of having two different $\theta$ for the two market models is complicated and unrealistic. On the other hand, we want to investigate this particular model setting  in order to clarify some mathematical aspects which were raised in Section \ref{sec_linear_TIM} (see remark \ref{os_two_theta}),
regardless of its economic meaning. 
}
In contrast to the previous section we start by specifying a particular transient impact function $G_2(t)$ in the secondary market model and we search for the suitable parameter setting of the primary market model so that the selected decay kernel are the corresponding intrinsic impact function, i.e., $G_2(t)\equiv G_{intr}(t)$.
{\color{blue} In other words, given $\bm{\eta}^*_{direc}$ we search a suitable parameter setting for the market impact game such that $\bm{\xi}^*_{direc}=\bm{\eta}^*_{direc}$.}


 \subsubsection{Linear Decay Kernel}
If $G_{2}^{pol}(t)= bt+c$ then for an equidistant time grid, $t_i=i/N, \ 
i=0,1,\ldots,N$,
$\Gamma_{i,j}=\frac{b|i-j|}{N}+c$. The inverse of $\Gamma$
is given by, see
\cite{dow2002explicit},
\[
\Gamma^{-1}=
\frac{1}{2b}
\begin{bmatrix}
-\eta_{N}/\eta_{N+1} & 1 & 0 &\cdots & 0 & b^2 /\eta_{N+1} \\
1& -2 & 1 &0 &\cdots &0 \\
0& 1 & -2 &1 & 0 & 0 \\
& & \ddots & \ddots & \ddots & \\
0&\cdots & 0 &1 &-2 &1\\
b^2 /\eta_{N+1} & 0 &\cdots &0 &1 &-\eta_{N}/\eta_{N+1}
\end{bmatrix}
\]
where $\eta_N=2cb+b^2(N-1)$. Then, $\Gamma^{-1} \bm{e}=[\star_1, \cdots, \star_1]^T$, so the $\bm{\eta}_{direc}^*=\frac{X_{direc}}{\bm{e}^T\Gamma^{-1} \bm{e} }
\Gamma^{-1} \bm{e}=[X_{direc}/2,0,\cdots,0 , X_{direc}/2]^T$ 
regardless of any choice of $b$ and $c$.

 \subsubsection{Exponential Decay kernel}
Let $G_{2}^{exp}(t)= \exp(-\rho t)=q^{-Nt}$, where $q=\exp(-\rho/N).$ Thus, the 
matrix $\Gamma$ is a  Kac-Murdock-Szegö (KMS) matrix, see \cite{dow2002explicit}, and it 
 has a simple tridiagonal inverse provided by
\[
\Gamma^{-1}=
\frac{1}{1-q^2}
\begin{bmatrix}
1 & -q & 0 &\cdots & 0  \\
-q& 1+q^2 & -q & \cdots &0 \\
 & \ddots & \ddots & \ddots & \\
0&\cdots & -q &1+q^2 &-q\\
0  & \cdots &0 &-q &1
\end{bmatrix},
\]
so that $ \Gamma^{-1} \bm{e}=\left[\frac{1}{1+q}, \frac{1-q}{1+q}, \cdots, \frac{1-q}{1+q}, \frac{1}{1+q}\right]^T$, i.e.,
the optimal schedule is to concentrate all the orders at the extremes and than to trade with constant rate in the mid trading times.
In particular, when $N\to \infty$ it
converges to two Dirac at the extremes like
 in \cite{Obizhaeva}, but more surprisingly it converges to 
 the solution provided by any linear transient impact model!
 This, means that when $N\to \infty$, the linear and the exponential intrinsic decay kernel, $G_{2}^{pol}(t)$ and $G_{2}^{exp}(t)$, 
 are equivalent, we discuss this point in the next section.
 
 \subsubsection{Power-law Kernel}
 Unfortunately, there is no a closed formula for 
 $\Gamma^{-1}$,
 when the decay kernel is a  power-law. However, if 
 $G_{2}^{pow}(t)=\frac{1}{(1+t)^{1-p}}$, Figure \ref{fig_power_law}
 illustrates the optimal schedule 
 $\frac{1}{\bm{e}^T\Gamma^{-1} \bm{e} }
\Gamma^{-1} \bm{e}$ for some\footnote{Trivially, when $p=1$ the solution does not exists since $\Gamma$
becomes singular.} $p>0$.
The solution has two peaks at the beginning and at 
the end of the session, while it decreases until it reaches a minimum in the middle, and
it is evident that the optimal solution is not 
constant between $t_1$ and $t_N$, see the inbox of 
Figure \ref{fig_power_law}, differently from what happens for the linear and exponential kernel. \\



      \begin{figure}[t]
\centering
{\includegraphics[width=0.85\textwidth]{plot_new/tim_sol_theta0_power_law.eps}}
\caption{  
Optimal schedule time for TIM when $\theta=0$
and the decay kernel is a power-law. 
The inbox figure displays the solution for the 
mid-time, i.e., between $t_1=\frac{1}{N}$ and 
$t_N=1-\frac{1}{N}$.
} 
\label{fig_power_law}
\end{figure}
 
 
 
 In conclusion when $\theta_2=0$ in the secondary market impact model, the optimal schedules are generically given by a vector who concentrates the orders at the 
 two extremes of the trading session and it has a constant trading rate for all mid trading times. So, the question is whether the solution of 
 a market impact game of the primary market model has a shape which looks like the one described above for the
 secondary market model (single-agent TIM).   
This is discussed in the following example, where another 
feature of the identification problem arise even if we assume that the two market impact models have different transaction cost levels.

%  \subsection{Uniqueness of the Intrinsic Market Impact Function}

 
 \begin{es}
 \label{es_theta0}
As already mentioned, in a generic TIM with $\theta_2=0$,
the linear and  exponential decay kernel generates the same optimal solution
when $N\to \infty$.
However, as showed in \cite{schied2017high}, the continuous time
Nash equilibrium of a general market impact game exists only for $\theta_1=\theta_1^*=G(0)/4$, where $G(t)=e^{-\rho t}$, and it coincides with the high-frequency limits ($N\to \infty$) of the discrete-time
equilibrium.

Therefore, inspired by the evidence of \cite{schied2017high}, we set $\theta=G_1/4$ for the primary market model.
 We observe that when $\theta_1=G_1/4$,  
 $\Gamma_{\theta_1}=2\theta_1 I+ G_1 \bm{e}\bm{e}^T=
 \frac{G_1}{2} I+G_1\bm{e}\bm{e}^T$ and so 

 \[ 
 (\Gamma_{\theta_1}+\widetilde{\Gamma})=
 G_1\begin{bmatrix}
 2 & 1 & 1 & \cdots &1\\
 2 & 2 & 1 &\cdots &1\\
 \vdots & & \ddots & &\vdots\\
  2 & & \cdots & 2 &1  \\
 2 & &\cdots &\cdots & 2  \\
 \end{bmatrix}, 
  (\Gamma_{\theta_1}+\widetilde{\Gamma})^{-1}=
G_1^{-1}\begin{bmatrix}
 1 &   &  & & -1/2 \\
 -1 & 1 &  \\
   & & \ddots & \ddots& \\
   & &  &-1 & 1  \\
 \end{bmatrix}
 \]
 
  \[ 
 (\Gamma_{\theta_1}-\widetilde{\Gamma})=
 G_1\begin{bmatrix}
 1 & 1 &  & \cdots &1\\
   & 1 &  &\cdots &1\\
  & &  &\ddots &\vdots\\
   & & & & 1  \\
 \end{bmatrix}, 
  (\Gamma_{\theta_1}-\widetilde{\Gamma})^{-1}=
G_1^{-1}\begin{bmatrix}
 1 &  -1 &   \\
  &  \ddots  &\ddots \\
   & &  1 &-1 \\
   & &   & 1  \\
 \end{bmatrix}.
 \]
 Therefore, $\bm{v}=[1, 0, \cdots, 0]^T$ and $\bm{w}=[0, \cdots ,0 ,1]^T$
 and the solution for the Directional $\bm{\xi}_{direc}^*$ in the primary market model
 is exactly equal to the one obtained by the secondary market model with no transaction cost and linear decay kernel, i.e., 
 $[X_{direc}/2, 0,\cdots,0 , X_{direc}/2]^T$.
Thus, any linear decay kernel $G_2^{pol}(t)$ can be selected as 
the intrinsic transient impact function $G_{intr}(t)$ when $\theta_1=\theta_1^*$ in the primary market model.
\end{es}

In general, under the above setting, we search the setting 
such that \\ $\bm{\xi}_{direc}^*=[X_{direc}/2,0,\cdots,0 ,
X_{direc}/2]^T$. Thus, the following result holds.

\begin{pr}\label{prop_xi_spikes}
In the market impact game of the primary market model,
$\bm{\xi}_{direc}^*=[X_{direc}/2,0,\cdots,0 , X_{direc}/2]^T$ if and only if $\theta_1=G_1/4$.
\end{pr}
\begin{proof}[Proof of Proposition \ref{prop_xi_spikes}]
From Example \ref{es_theta0} If $\theta_1=G_1/4$ then the Nash equilibrium of the market impact game is given by $\bm{\xi}_{direc}^*=[X_{direc}/2,0,\cdots,0 , X_{direc}/2]^T$.
Vice-versa, using the characterization of the Nash equilibrium, 
see Proposition \ref{direc_solut_symm} and Theorem \ref{NE_symm}, 
$\xi_{direc,1}^*=\frac{X_0}{2} \cdot \frac{(1+a^N)}{\lambda(1-a^{N+1})}$, where $a=1-1/\lambda$ and 
$\lambda=\frac{2\theta_1}{G_1}+\frac{1}{2}$, where $\theta_1\geq G_1/4$ so $a\in [0,1)$.  Thus, if $\xi_{direc,1}^*=X_0/2$, then 
$1+a^N=\frac{1-a^{N+1}}{1-a}\iff 1+a^N=1+a+a^2+\cdots +a^N\iff
0=a+a^2+\cdots +a^{N-1}$, so $a=0$, i.e., $\theta_1=G_1/4.$
\end{proof}
Therefore, when $\theta_2=0$ the intrinsic transient impact function is linear if and only if $\theta_1=G_1/4$, and in particular all linear decay kernel functions are  
solution of the intrinsic decay kernel problem, i.e., $\bm{\xi}_{direc}^*=\bm{\eta}_{direc}^*$ for all $G_{intr}(t)$ linear, see Example \ref{es_theta0}.
We observe that the same results can be obtained by using the same reasoning of Section \ref{sec_linear_TIM}.
Indeed, assuming a linear intrinsic decay kernel, i.e., using the notation of Section \ref{sec_linear_TIM}, $g_k=\alpha+\beta\frac{k}{N}$,  if we set $\theta=0$ and if
if $\bm{\xi}_{direc}^*=[X_{direc}/2,0,\cdots,0 , X_{direc}/2]^T$,
then for any $\beta$ it holds 
that $\Pi\bm{\xi}_{direc}^*=1$.
Furthermore, subtracting each member, we recover from the 
first two equations of $\Pi\bm{\xi}_{direc}^*=1$, that
$\beta(-\xi^*_{direc,1}+\sum_{k=2}^{N+1} \xi^*_{direc,k})=0$.
Therefore, in general if $\xi^*_{direc,k}>0$ for all $k$, then necessary $\beta=0$, which is however not admissible since the kernel matrix $\Gamma$ is singular, so the kernel cannot be linear.{\color{red}
Mi rendo conto che quest'ulitmo discorso è un po' contorto da spiegare. In realtà un po' tutta questa sezione...
}
 
\subsection{Transaction Costs Effect}\label{transaction_cost_effect}
 
 We now conclude this section by addressing the following question:
how does the impact of transaction costs affect the 
intrinsic transient decay kernel in market impact game?
Let us consider the same setting as in 
Section \ref{market_impact_game}, where the two market models 
have the same $\theta$. 
We focus on the linear intrinsic transient impact function.
From Section \ref{sec_linear_TIM} we known that the slope coefficient is provided by $ -\frac{4\theta N G_1^2}{16\theta^2-G_1^2}$. So, the absolute value of the slope is a decreasing function of $\theta$ which goes to zero for large values of $\theta$.
% Then, we estimate a linear decay kernel as intrinsic transient impact function in the secondary market, i.e. $G_{intr}^{pol}(t)=b t +c$, for different values of transaction costs levels $\theta$ (We assume the same 
% $\theta$ for the primary and secondary market impact game, as in section \ref{market_impact_game}).
% For all values of $\theta$s the estimates of the slope $b$ are statistically significant. Moreover,
% we observe that the absolute value of the slope $b$ is a decreasing function of $\theta$, see Figure \ref{fig_slope}.
%       \begin{figure}[t]
% \centering
% {\includegraphics[width=0.85\textwidth]{plot_new/slope_theta.eps}}
% \caption{ Estimates of the slope $b$ in function of transaction costs $\theta$ for a TIM where the decay kernel is linear, $G(t)^{TIM}=bt+c$.} 
% \label{fig_slope}
% \end{figure}
This may be also explained by looking the interaction between the two agents in the primary market model.
Indeed, when transactions costs increase this interaction between agents in market impact game disappears. In particular, when the 
transaction costs level is huge, the arbitrageur
gradually reduces the volume traded so that the optimal
schedule of the directional becomes as in the standard Almgren-Chriss framework, see Figure \ref{fig_sol_AC_theta}.
Therefore, there is no more interaction between the agents when $\theta$ increases and then the evidence of an intrinsic transient impact function 
vanishes.


     \begin{figure}[!t]
\centering
{\includegraphics[width=1.05\textwidth]{plot_new/sol_ac_fund_arbi_theta_varying.eps}}
\caption{Nash equilibria of market impact games in the primary market model with fixed $G_1=1$, and equidistant time grid where $T=1, N=25$, when the transaction costs level $\theta$ increases.} 
\label{fig_sol_AC_theta}
\end{figure}

\section{Multi-Asset Primary Market Model}

Until now we have considered a primary market model as 
a \cite{schied2018market} market impact game with $G_1=1$, where the two agents are risk neutrals and they trade the same (one) asset.
In this section we generalize this last conditions, and we consider the 
possibility that the two traders may 
liquidate a portfolio of $M$ assets.
In particular, 
we use the same framework modeling of \cite{cordoni2020instabilities}
to investigate also the relation between cross-impact effects
and the intrinsic decay kernel function.
In \cite{cordoni2020instabilities} it showed that for 
a Directional agent who wants to trade only one of the available assets,
it is in general convenient to trade also the other assets with a zero inventory condition due the cross-impact effects.
Therefore, we extend the previous analysis in the following way
In the primary market model we consider two risk-neutral agents, 
a Directional and an Arbitrageur who may trade $M$ assets, e.g., the inventory of the Directional may be $1$ for one asset and zero for the others.
% Without loss off generality, we may assume $\bm{X}_{direc}=(1,0,\ldots,0)^T\in \R^M$. 
We use the same model setting as above for
the secondary market model, i.e., we have only the Directional trader and the asset that he/she has to liquidate or buy.
As usual, we assume a constant decay kernel for the primary market model, $G_1=1$, and a general propagator function, $G_2(t)$ for the secondary one.
\subsection{Nash Equilibrium for the Primary Market Model}

The existence and uniqueness of Nash Equilibrium of the primary market model is guaranteed under general assumptions by the results of  \cite{cordoni2020instabilities}.{\color{blue}
bisognerebbe mostrare il risultato nostro nel caso in cui G è costante. Nel caso J=2 e gamma=0, dovrebbe essere semplice avere il risultato  anche per G=1. Nel caso generale (luo schied ) non mi sembra banale. L'argomentazione di sotto potrebbe bastare?
che ne pensi?
}
However, it is required that the decay kernel must be strictly definite positive in the sense of Bochner. Therefore, we may not apply directly their results when $G_1>0$ is constant.
On the other hand, the affected price process is described by
\[
   \bm{S}_t^{\Xi}= \bm{S}_t^0 -\sum_{t_k <t} G_1 Q(\bm{\xi}_{1,k}+\bm{\xi}_{2,k}), 
   \quad \forall\ t \in \numberset{T},
\]
where $\bm{S}_t^0\in \R^M$ is the unaffected price process and $\bm{\xi}_{i,k}\in \R^M$ is the 
vector of agent $i$ in the $M$ assets at time step $k$ and $Q\in \R^{M\times M}$ is the cross-impact matrix which is assumed to be (symmetric) and positive definite. If $Q$ is diagonal it is straightforward to obtain the Nash equilibrium from the Schied and Zhang equilibria for the $M$ assets
following the same reasoning of Section \ref{sec_ne_primary_model}
for each asset.  In the general case we may use the same argument of \cite{cordoni2020instabilities} to obtain 
the equilibria for the orthogonalized assets with respect to $Q$, i.e., 
using the spectral decomposition of $Q=VDV^T$, where V and D are the orthogonal and diagonal matrices
containing the eigenvectors and eigenvalues of $Q$, we may rewrite the affected price process in such a way the cross-impact matrix becomes diagonal multiplying by $V^T$. We may assume that 
the $D=\mbox{diag}(\lambda_1,\lambda_2,\ldots,\lambda_M)$ where 
$\lambda_i\geq\lambda_j$, for $i<j$.
Therefore, for each orthogonalized asset we may compute the related Nash equilibrium as for the one-asset in case of Section \ref{sec_ne_primary_model}. Finally, following \cite{cordoni2020instabilities} we may consider the linear combination of the Nash equilibria for the ortogonalized assets using the inverse transformation $V$. We observe that the same results can be generalized when we have $J$ risk-neutrals agents. 
Therefore, we may compute the Nash equilibrium in the multi-asset case using the formula provided by \cite{cordoni2020instabilities} when $G_1>0$ is constant. As for the previous setting we set the transaction costs $\theta$ in order to avoid the possibility of instabilities in the equilibria, see \cite{cordoni2020instabilities} for further details.
%caso G1=1, diagonalizzo i prezzi, poiché gamma=0 Q ortogonale il funztionale da minimizzare diventa la somma, quindi il NE diventa esattamente caratterizzato dalla combinazione dei NE ottenuti su i problemi ortogonali

We denote $\bm{X}_{direc}, \ \bm{X}_{arbi}\in \R^M$ the 
inventories related to the Directional and Arbitrageur, respectively.
We refer to the previous setting as a \emph{Schied and Zhang multi-asset market impact game}, where the two agents are risk-neutrals and the market impact is constant $G_1>0$.
Thus, the following results holds.
\begin{pr}
In a Schied and Zhang multi-asset market-impact game where the two agents are a 
Directional and an Arbitrageur, the Nash Equilibrium is time symmetric, i.e., 
\begin{align}\label{eq_symm_NE}
\bm{\xi}_{direc,k}^*&=\bm{\xi}_{direc,N+2-k}^*, \ k=1,2,\cdots,N+1,  \\
\bm{\xi}_{arbi,k}^*&=-\bm{\xi}_{arbi,N+2-k}^*, \ k=1,2,\cdots,N+1. 
\label{eq_symm_NE_2}
\end{align}
\end{pr}

\begin{proof}
As observed previously, we may use
Theorem 3.7 of \cite{cordoni2020instabilities} 
to compute the Nash equilibrium even if $G_1>0$.
Indeed, we first recover the transformed inventory using the eigenvectors matrix $V$ of $Q$, i.e., $\bm{X}^P_{direc}=V^T\bm{X}_{direc}$ and 
$\bm{X}^P_{arbi}=V^T\bm{X}_{arbi}$. We observe that since 
$\bm{X}_{arbi}=\bm{0}$ then $\bm{X}_{arbi}^P=\bm{0}$. So, 
for the orthogonalized problem, when the cross-impact is diagonal,
we have exactly $M$-stacked Schied and Zhang market impact where 
for each asset the market impact is constant to $G_1 \cdot \lambda_i$, where $\lambda_i$ is the corresponding $i$-th eigenvalue.
Therefore, the associated equilibrium for each 
orthogonalized asset $i$, $\bm{\xi}^P_{direc,\cdot,i}$
and $\bm{\xi}^P_{arbi,\cdot,i}$ can be obtained by Theorem \ref{NE_symm} where the fundamental solutions, $\bm{v}_i$ and 
$\bm{w}_i$ for each orthogonalized asset $i$ are computed using the 
adjusted decay kernel $G_1 \lambda_i$. Therefore, 
$\bm{\xi}^P_{direc,\cdot,i}$
and $\bm{\xi}^P_{arbi,\cdot,i}$ have a U-shape for all $i$ for Corollary \ref{cor_Ushape}. 
On the other hand, using the inverse transformation, $V$, we may recover the Nash equilibrium for the original non orthogonalized game, i.e., if $\Xi_j^{*,P}\in \R^{M\times (N+1)}$ denotes the matrix where each row $i$ corresponds to $\bm{\xi}^P_{j,\cdot,i}\in \R^{N+1}$ for agent $j$, then the Nash equilibrium $\Xi_j^{*}=V \Xi_j^{*,P}$.
Therefore, the optimal volume schedule for agent $j$ at time step $k$ for the asset $i$ is provided by 
$$\xi_{j,i,k}=\sum_{l=1}^M v_{i,l}\cdot \xi_{j,l,k}^P,$$
where $v_{i,l}$ the  $i$-th element of the $l$-th eiegenvector of $Q$.
Thus, since $\xi_{j,l,k}^P=\xi_{j,l,N+2-k}^P$, for each asset $l$ and
agent $j$, we conclude that $\xi_{j,i,k} =\xi_{j,i,N+2-k}$, for $k=1,\ldots,N+1$, i.e., the optimal schedule it is time symmetric. 
\end{proof}
In particular, the optimal schedule for agent $j$ at time step $k$ for the asset $i$ is provided by
$\xi_{j,i,k}=\sum_{l=1}^M v_{i,l}\cdot \xi_{j,l,k}^P$, 
where $v_{i,l}$ is the $i$-th element of the $l$-th eiegenvector of $Q$ and $\xi_{j,l,k}^P$ is the optimal schedule for the orthogonalized game where the cross impact is diagonal, corresponding to the eigenvalues of $Q$ for each asset, obtained by using the fundamental solutions
$\bm{v}_i$ and 
$\bm{w}_i$ computed using the decay kernel $G_1 \lambda_i$.
Even if, the time symmetric property does not depend in general on the 
spectral decomposition of $Q$ and on the inventory of the fundamentalist, the other property which characterize U-shape profile
of the optimal schedule might be not satisfied. Indeed, they convexity property may depend on the particular eigenvectors components of $Q$. {\color{blue}Ti torna questo discorso?}

On the other hand, if 
the Directional trader has inventory equal to one of the eigenvectors\footnote{In other words,
the Directional trader wants to liquidate or buy a market factor following a precise market signals,
if we interpret the eigenvectors of $Q$ as market factors .}
of $Q$, $\bm{v}_i$, then his/her inventory on the ortoganalized asset
is equal to the $i$-th element of the canonical base, i.e., 
the vector with one in position $i$ and zero otherwise.
This implies that with an exception of the orthogonalized asset 
$i$, the Nash equilibrium is zero, $\bm{\xi}^P_{direc,h,\cdot}=\bm{0}$ for $h\neq i$, since the two agents have zero
(orthogonalized) inventories for $h\neq i$.
Therefore, for an asset $h$,
the optimal schedule for agent $j$ at time step $k$ simplifies as
$\xi_{j,h,k}=\sum_{l=1}^M v_{h,l}\cdot \xi_{j,l,k}^P=
 v_{h,i}\cdot \xi_{j,i,k}^P
$, i.e., it is a rescaled version of the U-shape profile  
$\xi_{j,i,k}^P$ by the $h$-element of the $i$-th eigenvector of $Q$.
In particular, in this case we have the same evidence obtained for the one-asset case in Section \ref{sec_numerical_fit}, since the Nash equilibrium for each asset satisfies the relation \eqref{cond_linear_decay}.
% As an example we consider a primary market model
% with two asset, $M=2$ where the cross-impact matrix is given by 
% $$
% Q=\begin{bmatrix}
% 1 & 0.6\\ 0.6 & 1
% \end{bmatrix},
% $$
% $T=1$, $N=25$, $\theta=1$, $G_1=1$. 
% If the Directional has inventory equal to $(1\ 1)^T$ then its Nash equilibrium has a U-shape, since $(1\ 1)^T$ is an eigenvector of $Q$. 

In conclusion, in the multi-asset case when the Directional trader liquidate a position proportional to one of the market factors 
represented by the eigenvectors of $Q$, then the evidence of a transient market impact propagator function provided by the market impact game when the impact is set to a constant still remains as for the one asset case.
We conclude by briefly discussing the general case of multi-agent
market impact game.

\subsection{The Multi-Agent Case}\label{sec_multi_agent}
If we consider a multi-asset primary market model with $J>2$ agents, we may use the results of \cite{luo_schied} and \cite{cordoni2020instabilities} to recover the related Nash equilibria of agents. However, even in the one asset case, the results of Section \ref{sec_ne_primary_model} are no more valid 
when we consider $J>2$ traders in the primary market model,
 since the fundamental solutions depend on the number of agents which implies that the decay kernel matrix are no more Toeplitz in general, see e.g., \cite{luo_schied}. 
As an example we consider $2$ Arbitrageur and a Directional (risk-neutrals) traders, where they trade the same asset.
Figure \ref{fig_3_agents_NE}
exhibits the related Nash equilibria for the agents when 
we set $T=1$, $N=25$, $G_1=1$, $\theta=1$. 
We observe that the solutions of the two Arbitrageurs are identical.
Even if for the Arbitrageur the optimal solution is 
always a round-trip strategy facing the same direction of the Directional trader at the beginning of the session,
it is quite evident that the optimal solution for the Directional is a U-shape which is no more time-symmetric. In particular, it is optimal for him/her 
to trade more at the end of session exploiting the impact of the Arbitrageur.
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{plot_new/multi_agent_primary.eps}
    \caption{Nash equilibria for the primary market model with a Directional trader and two Arbitrageur, where 
    $T=1$, $N=25$, $G_1=1$, $\theta=1$. The solution of the two Arbitrageurs are identical.}
    \label{fig_3_agents_NE}
\end{figure}

%fare plot e dopo approccio alternativo

\section{Alternative Approach based on Price Dynamics}

We conclude by presenting an alternative approach to 
find evidence of transient market impact, regardless the shape 
of the Nash equilibrium.

Our previous approach has been to try to identify which kernel of the TIM model gives the same
optimal execution as the Nash equilibrium of a Schied-Zhang game.
Unfortunately it seems that there are two main problems: (i) the solution is not in general unique and (ii)
the question cannot be extended to the case with more than two agents (or one arbitrageur).

An alternative approach is to look at the (average) price dynamics, assuming the trading strategy
is the equilibrium one, rather than to the optimal execution. Remind that the price dynamics on a given trading time grid 
$\T=\{t_0,t_1,\ldots,t_N\}$ is described by
\[
S_t^{\Xi}=S_t^0-\sum_{t_k <t} G(t-t_k)(\xi_{1,k}+\xi_{2,k}),
\]
where $S_t^0$ is a right-continuous martingale defined on a given probability space which acts as volatility term. Therefore, if we discard the noise due to volatility, the above relation holds
between the expected value of price increments and order flow.
Thus, if $S_0=S_0^0$,
\[
\overline{S}_t^{\Xi}-S_0=-\sum_{t_k <t} G(t-t_k)(\xi_{1,k}+\xi_{2,k}),
\]
where $\overline{X}$ denotes the expectation of $X$, which can be recasted in a matrix form,
\begin{equation}\label{eq_alternative_system}
    \bm{S}=-\Gamma \bm{\Xi},
\end{equation}
where $\bm{S}=(\overline{S}_{t_0}^{\Xi}-S_0,\ldots, \overline{S}_{t_N}^{\Xi}-S_0)$
 is the aggregate drift, $\bm{\Xi}=\bm{\xi}_1+\bm{\xi}_2=
(\Xi_1,\ldots,\Xi_{N+1})^T$ is the aggregate order flow and 
\[
\Gamma=
\begin{bmatrix}
G(0) & 0 & 0 & \cdots  &\cdots   &0\\
G(1) & G(0) & 0 & 0&  \cdots  &0\\
G(2) & G(1) & G(0) & 0& \ddots & 0\\
\vdots & \ddots &\ddots  & \ddots & \ddots &\vdots\\
G(N-1) & G(N-2) &\cdots  &\cdots   & G(0) & 0  \\
G(N) & G(N-1) & G(N-2)&   \cdots &  \cdots& G(0)  \\
\end{bmatrix}.
\]
However, we may rewrite the above system as $\bm{S}=-M \bm{g}$, 
where $\bm{g}=(G(0),G(1),\ldots,G(N))^T$
and 
\[
M=
\begin{bmatrix}
\Xi_1 & 0 & 0 & \cdots  &\cdots   &0\\
\Xi_2 & \Xi_1 & 0 & 0&  \cdots  &0\\
\Xi_3 & \Xi_2 & \Xi_1 & 0& \ddots & 0\\
\vdots & \ddots &\ddots  & \ddots & \ddots &\vdots\\
\Xi_N & \Xi_{N-1} &\cdots  &\cdots   & \Xi_1 & 0  \\
\Xi_{N+1} & \Xi_N & \Xi_{N-1}&   \cdots &  \cdots& \Xi_1  \\
\end{bmatrix}.
\]
If the aggregate net order flow is different from zero at $t_0$, i.e., $\Xi_1\neq0$, the matrix $M$ is non singular
and therefore there is always an unique solution which from the price dynamics
gives the order flow, 
\begin{equation}\label{eq_defi_alter_intrinsic_decay_kernel}
    \bm{g}=-M^{-1}\bm{S}
 \end{equation}
from which we recover the kernel $G$.

Thus, one could use $\bm{\xi}_1$ and $\bm{\xi}_2$, the Nash equilibrium solution of Schied and Zhang with linear
kernel and obtain $S$,  from Equation \eqref{eq_alternative_system}. Then, assuming only one agent (the Directional, say agent 1)
is present in a TIM, i.e., the secondary market model, one solves Equation \eqref{eq_defi_alter_intrinsic_decay_kernel} using for the order flow 
$\Xi=\bm{\xi}_1$ and finds the intrinsic decay kernel.
Equation \eqref{eq_defi_alter_intrinsic_decay_kernel} is an alternative definition to Definition \ref{def_intrinsic_decay_kernel}  of the intrinsic transient impact function, which we emphasise in the following definition.


\begin{de}\label{intrinsic_def_2}
(Intrinsic  transient  impact  function -  Alternative Def.). The  transient  impact  function $G_{intr,2}(t)$  which satisfies 
$\bm{S}=-M \bm{g}$, where $M$ depends on $\bm{\xi}_1$ and $\bm{S}$ is recovered by the aggregate (drift) order flow of the primary market model $\Xi$,  is  called \emph{intrinsic transient impact function}.
\end{de}
In contrast to Definition \eqref{def_intrinsic_decay_kernel}
the intrinsic decay is now uniquely identified, which
is true both for the Schied and Zhang game and for the TIM. Even
for the Schied and Luo game with many agents there will be a unique solution for $G_{intr,2}(t)$.
However, it is straightforward that using this definition we can not use the intrinsic decay kernel to solve the TIM optimal solution problem and recover the previous relation between Nash equilibrium and optimal schedule of a TIM.
Since $\Xi_1\neq0$, we can not consider the case when the number of buyer Directional is the same of the seller one (on the same assets), otherwise their aggregate orders are equal to zero.

\begin{os}
To be precise, if we consider the equally spaced time grid $0=t_0<t_1\cdots<t_N=T$ at trading time  $t_k$ 
the order $\Xi_{k+1}$ arrives and

$$
S_{t_k}^{\Xi}=S_{t_k}^0-\sum_{h=0}^{k-1} G(t_k-t_h) \Xi_{h+1},
$$
therefore, since $S_{t_0}^{\Xi}=S_{t_0}^0$
at time $t_{0+}$ such that 
$t_0<t_{0+}<t_1$, then the price is moved from $S_{t_0}$ to  $S_{t_{0+}}$, where 
$S_{t_{0+}}^{\Xi}=S_{t_0}^0-G(0)\xi_1$
Thus, we have to consider the ``artificial" trading time $t_{k+}$ in 
system \eqref{eq_alternative_system}.
\end{os}

We first consider the same setting of Section \ref{sec_non_param_fitting}, where in the primary market model 
there are the Directional and one Arbitrageur and the decay kernel is set to $G_1(t)\equiv1$. 
We then compute the cumulative drift  $\bm{S}$ generated by the interaction of the two agents, then we solve system \eqref{eq_defi_alter_intrinsic_decay_kernel} where $M$ is computed by considering only the drift generated of the Directional $\bm{\xi}_{Direc}$ and 
we report in Figure \ref{fig:alternativeSZ} the intrinsic transient impact function $G_{intr,2}(t)$. 
Moreover, we compute $G_{intr,2}(t)$ when we consider a Luo and Schied game with $1$ Directional trader and $2$ Arbitrageurs using the same setting of Section \ref{sec_multi_agent}, where the decay kernel is set to $G_1(t)\equiv1$. 
We recall that the Nash Equilibrium in this case is non more time-symmetric, see Figure \ref{fig_3_agents_NE}.
It is quiet evident that the shape of $G_{intr,2}(t)$ is highly nonlinear for both settings. 
Qualitatively, we observe that the two intrinsic transient impact kernels seem differ in terms of ``size impact", i.e, the absolute value of $G_{intr,2}(0)$ is greater for the Luo and Schied game, 
but they exhibit the same shape. In particular they are both negative and qualitatively decreasing functions. 
Furthermore, since the cumulative drift $\bm{S}$ is generated by the interactions of the Fundamentalist and Arbitrageur(s), it converges (in absolute value) to the inventory of the Fundamentalist (1 in our example). Precisely, the aggregate order flow, due the 
symmetry of Nash equilibrium, decreases to zero since in the last trading times the Arbitrageur(s) and the Directional have opposite orders which compensate each other. 
Therefore, when we solve system \eqref{eq_alternative_system} considering only the impact of the Directional in the matrix $M$, 
we find a kernel which highlights how the impact order of the Directional 
is about $1/2$ and $1/3$, respectively for the two and three players games of the aggregate drift at time $t_0$.
\begin{figure}
    \centering
    \subfloat[][]
    {\includegraphics[width=0.48\textwidth]{plot_new/g_intr_schied.eps}}
       \subfloat[][]{\includegraphics[width=0.48\textwidth]{plot_new/g_intr_luo_schied.eps}}
    \caption{The intrinsic temporary impact function computed solving system \eqref{eq_defi_alter_intrinsic_decay_kernel} when we consider the cumulative drift generated by a Scied and Zhang game with a $1$ Directional trader and $1$ Arbitrageur, exhibit (a), and
    when we consider the cumulative drift generated by a Luo and Schied game with a $1$ Directional trader and $2$ Arbitrageur, exhibit (b).}
    \label{fig:alternativeSZ}
\end{figure}


\clearpage

 

==> sec_alternative_approach_backup_downgrade_21_01_2022.tex <==




%arrivato quis

%fare plot e dopo approccio alternativo

\section{Alternative Approach Based on Price Dynamics}
\label{sec_alternative_app}

We conclude by presenting an alternative approach to 
obtain evidence of transient market impact, regardless of the shape 
of the Nash equilibrium.

Our previous approach has been to try to identify which kernel of the TIM model gives the same
optimal execution as the Nash equilibrium of a market impact game.
Unfortunately, it seems that there are two main problems: (i) the solution is not in general unique and (ii)
the question cannot be extended to the case with more than two agents.

An alternative approach is to look at the (average) price dynamics.
%, where the trading strategies are assumed to be
%at the equilibrium, rather than to be optimal executions. 
Remind that the price dynamics on a given trading time grid 
$\T=\{t_0,t_1,\ldots,t_N\}$ is described by
\[
S_t^{\Xi}=S_t^0-\sum_{t_k <t} G(t-t_k)(\xi_{1,k}+\xi_{2,k}),
\]
where $S_t^0$ is a right-continuous martingale defined on a given probability space which acts as volatility term.
% {\color{blue}
% For the sake of simplicity we assume that $\T$ is an equidistant time grid}.
Therefore, if we discard the noise due to volatility, the above relation holds
between the expected value of price increments and order flow.
Thus, if $S_0=S_0^0$,
\[
\overline{S}_t^{\Xi}-S_0=-\sum_{t_k <t} G(t-t_k)(\xi_{1,k}+\xi_{2,k}),
\]
where $\overline{X}$ denotes the expectation of $X$, which can be recasted in a matrix form,
\begin{equation}\label{eq_alternative_system}
    \bm{S}=-C \bm{\Xi},
\end{equation}
{\color{blue} 
where $\bm{S}=(\overline{S}_{t_1}^{\Xi}-S_0,\ldots, \overline{S}_{t_{N+1}}^{\Xi}-S_0)$
 is the aggregate drift, $\bm{\Xi}=\bm{\xi}_1+\bm{\xi}_2=
(\Xi_1,\ldots,\Xi_{N+1})^T$ is the aggregate order flow and }
% \[
% C=
% \begin{bmatrix}
% G(0) & 0 & 0 & \cdots  &\cdots   &0\\
% G(1) & G(0) & 0 & 0&  \cdots  &0\\
% G(2) & G(1) & G(0) & 0& \ddots & 0\\
% \vdots & \ddots &\ddots  & \ddots & \ddots &\vdots\\
% G(N-1) & G(N-2) &\cdots  &\cdots   & G(0) & 0  \\
% G(N) & G(N-1) & G(N-2)&   \cdots &  \cdots& G(0)  \\
% \end{bmatrix}.
% \]
\[
C=
\begin{bmatrix}
G(t_1-t_0) & 0 & 0 & \cdots  &\cdots   &0\\
G(t_2-t_0) & G(t_2-t_1) & 0 & 0&  \cdots  &0\\
G(t_3-t_0) & G(t_3-t_1) & G(t_3-t_2) & 0& \ddots & 0\\
\vdots & \ddots &\ddots  & \ddots & \ddots &\vdots\\
G(t_{N}-t_0) & G(t_{N}-t_1) &\cdots  &\cdots   & G(t_{N}-t_{N-1}) & 0  \\
G(t_{N+1}-t_0) & G(t_{N+1}-t_1) & G(t_{N+1}-t_2)&   \cdots &  \cdots& G(t_{N+1}-t_{N})  \\
\end{bmatrix}.
\]
However,
we may rewrite the above system as $\bm{S}=-\mathcal{M} \bm{g}$, 
{\color{blue}
where in the case that $\T$ is an equidistant time grid.
$\bm{g}=(G(t_0),G(t_1),\ldots,G(t_{N}))^T$}
and 
\[
\mathcal{M}=
\begin{bmatrix}
\Xi_1 & 0 & 0 & \cdots  &\cdots   &0\\
\Xi_2 & \Xi_1 & 0 & 0&  \cdots  &0\\
\Xi_3 & \Xi_2 & \Xi_1 & 0& \ddots & 0\\
\vdots & \ddots &\ddots  & \ddots & \ddots &\vdots\\
\Xi_N & \Xi_{N-1} &\cdots  &\cdots   & \Xi_1 & 0  \\
\Xi_{N+1} & \Xi_N & \Xi_{N-1}&   \cdots &  \cdots& \Xi_1  \\
\end{bmatrix}.
\]
If the aggregate net order flow is different from zero at $t_0$, i.e., $\Xi_1\neq0$, the matrix $\mathcal{M}$ is non singular
and therefore there is always an unique solution
% which from the price dynamics
% gives the order flow, 
\begin{equation}\label{eq_defi_alter_intrinsic_decay_kernel}
    \bm{g}=-\mathcal{M}^{-1}\bm{S}
 \end{equation}
from which we recover the kernel $G$.

%{\color{blue} questa osservaizione non è più necessaria volendo.}
%\begin{os}
%To be precise, if we consider the equally spaced time grid $0=t_0<t_1\cdots<t_N=T$, at trading time  $t_k$ the order $\Xi_{k+1}$ arrives and
$$
S_{t_k}^{\Xi}=S_{t_k}^0-\sum_{h=0}^{k-1} G(t_k-t_h) \Xi_{h+1}.
$$
%Since $S_{t_0}^{\Xi}=S_{t_0}^0$ at time $t_{0+}$, where t_0<t_{0+}<t_1$, the price is moved from $S_{t_0}$ to  $S_{t_{0+}}$, where $S_{t_{0+}}^{\Xi}=S_{t_0}^0-G(0)\Xi_1$. Thus, we may repeat the same reasoning for trading time $t_k$, i.e.,$S_{t_{k+}}^{\Xi}=S_{t_k}^0-G(0)\Xi_{k+1}$. Therefore, we have to consider the ``artificial" trading time $t_{k+}$ in system \eqref{eq_alternative_system}.
%\end{os}

{\color{blue}
We now follow the same argument of the previous approach with a particular difference.
Thus, one could use $\bm{\xi}_1$ and $\bm{\xi}_2$, the Nash equilibrium solution of Schied and Zhang 
(e.g., using a linear constant decay kernel)
%with linear kernel 
and obtain the (equilibrium) price dynamics $\bm{S}$,  from Equation \eqref{eq_alternative_system}. 

Then, we ask the following question.
What is the impact faced by the only directional trader
when he does not consider the presence of other agents? 
Precisely, what is the propagator function inferred by the directional if she solves the optimal execution problem in the standard Almgren-Chriss framework? 
In this case, the market impact considered by the directional is the same as that of the MIG, i.e., it is constant, even if he does not take into account any other competitors.
This is a substantial difference with respect to the previous approach.
Thus, once derived the optimal execution for the directional, $\bm{\xi}_{AC}=\frac{X_0}{N+1}\bm{e}$, we wonder what the market impact inferred by the trader is. To answer this question, we solve the Equation \eqref{eq_defi_alter_intrinsic_decay_kernel}, where $\Xi=\bm{\xi}_{AC}$,
 so that we can obtain the intrinsic decay kernel associated with the single-agent characterized by the price dynamics of the market impact games.
 This leads to an alternative definition to Definition \ref{def_intrinsic_decay_kernel}  of the intrinsic transient impact function, which we emphasize in the following definition.
 
% Then, assuming only one agent (the directional, say agent 1)
% % which is present in a TIM (the secondary market model) one solves Equation  using the order flow of the directional, i.e.,  
% $\Xi=\bm{\xi}_1$,
% Equation \eqref{eq_defi_alter_intrinsic_decay_kernel} leads to an alternative definition to Definition \ref{def_intrinsic_decay_kernel}  of the intrinsic transient impact function, which we emphasise in the following definition.
}

\begin{de}\label{intrinsic_def_2}
(Intrinsic  transient  impact  function -  Alternative Definition). The  transient  impact  function $G_{intr,2}(t)$  which satisfies 
$\bm{S}=-\mathcal{M} \bm{g}$, where $\mathcal{M}$ depends on $\bm{\xi}_{AC}$ and $\bm{S}$ is recovered by the aggregate (drift) order flows, $\Xi$, of the market impact game  is  called \emph{intrinsic transient impact function}.
\end{de}


As previously shown,
in contrast to Definition \eqref{def_intrinsic_decay_kernel}
the intrinsic decay is now uniquely identified. 
We emphasize these results in the following theorem.

\begin{te}\label{te_alter_defin}
If the aggregate net order flow is different from zero at $t_0$, i.e., $\Xi_1\neq0$, the linear system $\bm{S}=-\mathcal{M} \bm{g}$ has unique solution for $\bm{g}$.
\end{te}

%, which
%is true both for the Schied and Zhang game and for the TIM.
Moreover,
even
for the Schied and Luo game with many agents there will be a unique solution for $G_{intr,2}(t)$.
However, it is straightforward that using this definition, we can not use the intrinsic decay kernel, $G_{intr,2}(t)$, to solve the TIM optimal solution problem and recover the previous relation between Nash equilibrium and optimal schedule of a TIM.
Since $\Xi_1\neq0$, we can not consider the case when the number of directional buyers is the same as the seller one (on the same assets), otherwise their aggregate orders will be equal to zero.



{\color{blue}
We first consider the same setting of Section \ref{sec_non_param_fitting}, wherein the primary market model there are the directional and one arbitrageur and the decay kernel is set to $G_1(t)\equiv1$. 
Then, we  compute the cumulative drift  $\bm{S}$ generated by the interaction of the two agents. We solve system \eqref{eq_defi_alter_intrinsic_decay_kernel} where $\mathcal{M}$ is computed by considering only the drift generated by the directional derived by the same model by without considering the presence of the arbitrageur, i.e., an 
Almgren and Chriss optimal schedule $\bm{\xi}_{AC}$ and 
we report in Figure \ref{fig:alternativeSZ} the intrinsic transient impact function $G_{intr,2}(t)$. 
Moreover, we compute $G_{intr,2}(t)$ when we consider a Luo and Schied game with $1$ directional trader and $2$ arbitrageurs using the same setting of Section \ref{sec_multi_agent}, where the decay kernel is set to $G_1(t)\equiv1$. 
We recall that the Nash Equilibrium, in this case, is non more time-symmetric, see Figure \ref{fig_3_agents_NE}.
The shape of $G_{intr,2}(t)$ is highly nonlinear for both settings. 

Qualitatively, we observe that the two intrinsic transient impact kernels seem to differ in terms of ``size impact", i.e., the absolute value of $G_{intr,2}(0)$ is greater for the Luo and Schied game than those obtained starting from the Schied and Zhang model, 
but they exhibit the same shape. In particular, they are both positive and qualitatively decreasing functions.
Moreover, solving Equation \eqref{eq_defi_alter_intrinsic_decay_kernel} we may derive that $G_{intr,2}(t_0)=(N+1)\cdot \Xi_1$, i.e., when we increase the frequency of the trading the price impact at $t_0$ increase accordingly.


The following motivation can interpret the shape of the fitted decay kernel.
Since the cumulative drift $\bm{S}$ is generated by the interactions of the fundamentalist and arbitrageur(s), it converges (in absolute value) to the inventory of the fundamentalist (1 in our example). Precisely,
due the symmetry of Nash equilibrium,
the aggregate order flow  decreases to zero since in the last trading times, the arbitrageur(s) and the directional have opposite orders which compensate each other, see Figure \ref{fig:alternativeSZ_2}.
This shape is obtained by setting a constant market impact. Therefore when we consider a constant order flow, like the one obtained by the Almgren and Chriss optimal schedule $\bm{\xi}_{AC}$, we derive a strictly decreasing market impact function with an appropriate scaling factor provided by
$G(t_0)=(N+1) \cdot \Xi_1$.
Moreover, since we set $G_1(t)$ to a constant, the aggregate volume traded is directly proportional to the price dynamics, see Figure \ref{fig:alternativeSZ_2} right panels.
% Therefore, when we solve system \eqref{eq_alternative_system} considering only the impact of the directional in the matrix $\mathcal{M}$, 
% we find a kernel which highlights how the order impact  of the directional 
% is about $1/2$ and $1/3$ of the aggregate drift at time $t_0$, respectively for the two, 
% (where $\bm{\xi}_{Direc,1}=\frac{\Xi_{1}}{2}$),
% and three, (where $\bm{\xi}_{Direc,1}=\frac{\Xi_{1}}{3}$), players games.


}
\begin{figure}[!t]
    \centering
    \subfloat[][]
    {\includegraphics[width=1\textwidth]{plot_new/g_intr_schied_2.eps}}\\
       \subfloat[][]{\includegraphics[width=1\textwidth]{plot_new/g_intr_luo_schied_2.eps}}
    \caption{The intrinsic temporary impact function computed solving system \eqref{eq_defi_alter_intrinsic_decay_kernel} when we consider the cumulative drift generated by a Schied and Zhang game with a $1$ directional trader and $1$ arbitrageur, exhibit (a), and
    when we consider the cumulative drift generated by a Luo and Schied game with a $1$ directional trader and $2$ arbitrageur, exhibit (b).}
    \label{fig:alternativeSZ}
\end{figure}


\begin{figure}[!t]
    \centering
    \subfloat[][]
    {\includegraphics[width=1\textwidth]{plot_new/g_intr_schied_2_interp.eps}}\\
       \subfloat[][]{\includegraphics[width=1\textwidth]{plot_new/g_intr_luo_schied_2_interp.eps}}
    \caption{Aggregate volume traded and its relation with price dynamics derived by a directional and an arbitrageur following the Schied and Zhang game and, panel (a), and by a directional and two arbitrageurs following a Luo and Schied game, panel (b).}
    \label{fig:alternativeSZ_2}
\end{figure}

 

==> sec_app_parametric_fit.tex <==

\clearpage
\section{Fitted Implied Transient Impact Functions}\label{sec_numerical_fit}

In this Appendix we investigate the possible families for $G_{intr}^{(P)}(t)$ by fitting the price impact in the optimal execution problem, in such a way $\bm{\eta}_{direc}^*$ matches the directional's schedule of
the market impact games $\bm{\xi}_{direc}^*$.
 

\subsubsection*{Non Parametric Fitting}\label{sec_non_param_fitting}

We try to fit $G_{intr}^{(P)}(t)$ in a non parametric  way. We only impose that the decay kernel must be convex and decreasing. 
% Since the kernel is identified up to a constant, we fix $G_{intr}^{(P)}(T)=0$.
We consider a market impact game model with an equidistant 
time grid $\T_N=\{\frac{kT}{N}| k=0,1,\ldots,N\}$, where
$T=1$, $N=25$, $G_1=1$, $\theta=1$.
The inventories of the two risk-neutral agents are equal to $1$ and $0$, respectively.
As observed by Remark \ref{up_constant}, the kernel is
identified up to a constant.
Thus, we impose 
for each fitted kernel that $G(T)=0$.
From Theorem \ref{te_linear_beta_results} we may 
identify the slope $\beta$ of the linear intrinsic decay kernel which is given by $\beta= -\frac{4\theta N G_1^2}{16\theta^2-G_1^2}=-6.6667$.
We start by selecting $100$ different starting points 
using 50 exponential and 50 power-law decay kernels.
Figure \ref{fig_non_par_fitting1} reports the starting points from the exponential and power-law decay kernels, panels (a) and (b), respectively, and the fitted 
intrinsic decay kernel.
The average error between $\bm{\xi}_{direc}^*$ 
and 
the fitted $\bm{\eta}_{direc}^*$ is $2.0938 e-05$.
Even if 
some fitted intrinsic decay kernel seems to be
nonlinear, we observe that all the fitted kernel seems to be close to the linear intrinsic decay kernel 
$-6.6667\cdot t+6.6667$.
We repeat the previous analysis by choosing different starting points. As before,
Figure \ref{fig_non_par_fitting2} reports the starting points from the exponential and power-law decay kernels, panels (a) and (b), respectively, and the fitted 
intrinsic decay kernel.
In this case the average error between $\bm{\xi}_{direc}^*$ 
and 
the fitted $\bm{\eta}_{direc}^*$ is $1.6226e-07$.
Moreover, all the fitted intrinsic decay kernel coincide, for almost all points, with the linear 
linear intrinsic decay kernel. 
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.4]{plot_new/fitted_decay_kernel_nonparam1.eps}
    \caption{First non parametric fitting. 100 starting points from the exponential and power law decay kernels, panels (a) and (b), respectively, and the fitted 
intrinsic decay kernel, right panel. The market impact game model has an equidistant time grid $T=1$, $N=25$, $G_1=1$, $\theta=1$.
The inventory of the two risk-neutral agents are equal to $1$ and $0$, respectively.}
    \label{fig_non_par_fitting1}
\end{figure}
\begin{figure}[!t]
\centering
    \includegraphics[scale=0.4]{plot_new/fitted_decay_kernel_nonparam2.eps}
    \caption{Second non parametric fitting. 100 starting points from the exponential and power law decay kernels, panels (a) and (b), respectively, and the fitted 
intrinsic decay kernel, right panel. The market impact game model has an equidistant time grid $T=1$, $N=25$, $G_1=1$, $\theta=1$.
The inventory of the two risk-neutral agents are equal to $1$ and $0$, respectively.}
    \label{fig_non_par_fitting2}
\end{figure}

From this analysis, the linear intrinsic decay kernel appears to be a privileged candidate as an intrinsic decay kernel. 
We did not find any particular evidence of other possible families of 
$G_{intr}^{(P)}(t)$. Thus, in next section we further investigate if the linear solution is the unique family of $G_{intr}^{(P)}(t)$ using parametric fitting.
Overall, even if we specify a family to the 
intrinsic decay kernel, the linear solution seems to be the unique solution that provides an appropriate fit. 
% We may 
% conjecture that the unique intrinsic decay kernel is actually the linear one discussed in Section \ref{sec_linear_TIM}.


\subsubsection*{Parametric Fitting}\label{sec_param_fitting}
 
We select three family to estimate the intrinsic decay kernel function:
\begin{itemize}
\item polynomial, $G_{intr}^{pol}(t)= \alpha_2 t^2+\alpha_1 t+\alpha_0$;
\item exponential $G_{intr}^{exp}(t)=\lambda e^{-\rho t}+\gamma$;
\item power law $G_{intr}^{pow}(t)=\frac{B}{(1+t)^{1-p}}+C$.
\end{itemize}

Then, we can easily fit the parameters from the
directional seller solution of a market impact game.  
% We assume momentarily that $\theta$ is the same for 
% both the market impact game and the single-agent TIM for the secondary market model. 
% In the next section we discuss how to relax this assumption.
We select the same setting as the previous subsection, an equidistant time grid where $T=1$, $N=25$, $G=1$, $\theta=1$ where we impose a constraint on the 
intercept terms $\alpha_0$, $\gamma$, $C$ such that $G_{intr}^{(P)} (T)=0$.


Table \ref{tab_fitted_kernel} exhibits the 
fitted parameters for the various decay kernel.
By comparing the residual sum of squares, the best fit is provided by the polynomial  family. The power law fitting provides nonsignificant estimate of the coefficient $B$. 
Moreover, the quality of the fit is very poor compared to the first two families.
We observe from Figure 
\ref{fig_decay_kernel} and \ref{fig_ne_ac_tim} that the most appropriate 
family is the linear one followed by the exponential decay, which is however
also very close to being linear.
In particular, it is quite evident that the solution provided 
by the power law family does not provide a good fit.


\begin{table}[t]
\centering
\caption{Fitted parameters for the three different intrinsic decay kernel families.
For each parameters it is reported the estimate, standard error and confidence interval at 95\%. Res.norm is 
the value of the squared 2-norm of the residual. The intercept term for each fitted kernel is selected in such a way that $G_{intr}^{(P)}(T)=0$}
\label{tab_fitted_kernel}
\begin{tabular}{lllll}
\toprule
    & Estimate            & SE       & CI 95\%    &            \\
    \midrule
    Polynomial\\
 $\alpha_2$ & -0.3671e-05 &   0.0867e-05 &  -0.5460e-05 &   -0.1881e-05  \\
 $\alpha_1$ & -6.6667  &  2.2622e-06  & -6.6667 &  -6.6667\\
Res.norm & 1.0641e-14\\
\midrule
  Exponential\\
 
$\lambda$ & 193.7472  & 38.5179 & 114.2502 & 273.2442\\
 $\rho$   & 0.0357   & 0.0074   & 0.0204  &  0.0509\\
 
Res.norm & 8.3847e-06 \\
\midrule 
Power-law\\
$p$ & 0.9954  &  0.2321  &  0.5163  &  1.4745  \\
   $B$ & 0.0288e05 &    1.4410e05 &  -2.9453e05 &   3.0029e05    \\
     Res.norm & 0.0026       \\
    \bottomrule
\end{tabular}
\end{table}


     \begin{figure}[t]
\centering
{\includegraphics[width=0.85\textwidth]{plot_new/fitted_kernel_param.eps}}
\caption{ The fitted decay kernel among the three selected 
family.} 
\label{fig_decay_kernel}
\end{figure}

     \begin{figure}[t]
\centering
{\includegraphics[width=0.85\textwidth]{plot_new/TIM_with_fitted_kernel_on_AC.eps}}
\caption{Nash equilibrium $\bm{\xi}_{direc}^*$ of the Directional
obtained from the market impact game with permanent impact (green), 
and 
Nash equilibrium $\bm{\eta}_{direc}^*$ for the optimal execution model with the fitted polynomial (cyan), exponential (blue) and power intrinsic decay kernel (red).
} 
\label{fig_ne_ac_tim}
\end{figure}



==> sec_multi_assets.tex <==

\section{Multi-Assets Primary Market Model}
\label{sec_mig_general}

Until now, we have considered a primary market model as 
a \cite{schied2018market} market impact game with $G_1=1$, where the two agents are risk-neutral and they trade the same (one) asset.
In this section, we generalize this last condition, and we consider the 
possibility that the two traders may 
liquidate a portfolio of $M$ assets.
In particular, 
we use the same framework modeling of \cite{cordoni2020instabilities}
to investigate also the relation between cross-impact effects
and the intrinsic decay kernel function.
In \cite{cordoni2020instabilities} it is showed that for 
a directional agent who wants to trade only one of the available assets,
it is generally convenient to trade other assets with a zero inventory condition due to the cross-impact effects.
Therefore, we extend the previous analysis in the following way.
In the primary market model, we consider two risk-neutral agents, 
a directional and an arbitrageur who may trade $M$ assets, where the inventory of the directional is $1$ for one asset and zero for the others.
% Without loss off generality, we may assume $\bm{X}_{direc}=(1,0,\ldots,0)^T\in \R^M$. 
We use the same model setting as above for
the optimal execution model, i.e., there is only the directional trader and the asset that the agent has to liquidate or buy.
Consistently with the previous setting, we assume a constant decay kernel for the primary market model, $G_1=1$, and a general propagator function, $G_2(t)$ for the secondary one.
\subsection{Nash Equilibrium for the Multi-Asset Primary Market Model}

The existence and uniqueness of Nash Equilibrium of the primary market model is guaranteed under general assumptions by the results of  \cite{cordoni2020instabilities}.
% {\color{blue}FC: 
% bisognerebbe mostrare il risultato nostro nel caso in cui G è costante. Nel caso J=2 e gamma=0, dovrebbe essere semplice avere il risultato  anche per G=1. Nel caso generale (luo schied ) non mi sembra banale. L'argomentazione di sotto potrebbe bastare?
% che ne pensi?
% }
However, it is required that the decay kernel must be strictly definite positive in the sense of Bochner. Therefore, we may not apply their results directly  when $G_1>0$ is constant.
On the other hand, the affected price process is described by
\[
   \bm{S}_t^{\Xi}= \bm{S}_t^0 -\sum_{t_k <t} G_1 Q(\bm{\xi}_{1,k}+\bm{\xi}_{2,k}), 
   \quad \forall\ t \in \numberset{T},
\]
where $\bm{S}_t^0\in \R^M$ is the unaffected price process and $\bm{\xi}_{i,k}\in \R^M$ is the 
vector of agent $i$ in the $M$ assets at time step $k$ and $Q\in \R^{M\times M}$ is the cross-impact matrix which is assumed to be (symmetric) and positive definite. If $Q$ is diagonal, it is straightforward to obtain the Nash equilibrium from the Schied and Zhang equilibria for the $M$ assets
following the same reasoning of Section \ref{sec_ne_primary_model}
for each asset.  In the general case we may use the same argument of \cite{cordoni2020instabilities} to obtain 
the equilibria for the orthogonalized assets with respect to $Q$, i.e., 
using the spectral decomposition of $Q=VDV^T$, where V and D are the orthogonal and diagonal matrices
containing the eigenvectors and eigenvalues of $Q$, we may rewrite the affected price process in such a way the cross-impact matrix becomes diagonal multiplying by $V^T$. We may assume that 
the $D=\mbox{diag}(\lambda_1,\lambda_2,\ldots,\lambda_M)$ where 
$\lambda_i\geq\lambda_j$, for $i<j$.
Therefore, for each orthogonalized asset we may compute the related Nash equilibrium as for the one-asset in the case of Section \ref{sec_ne_primary_model}. Finally, following \cite{cordoni2020instabilities} we may consider the linear combination of the Nash equilibria for the orthogonalized assets using the inverse transformation $V$. 
%We observe that the same results can be generalized when we have $J$ risk-neutrals agents. 
Therefore, we may compute the Nash equilibrium in the multi-asset case using the results provided by \cite{cordoni2020instabilities} when $G_1>0$ is constant. As for the previous setting, we set the transaction costs $\theta$ in order to avoid the possibility of instabilities in the equilibria, see \cite{cordoni2020instabilities} for further details.
%caso G1=1, diagonalizzo i prezzi, poiché gamma=0 Q ortogonale il funztionale da minimizzare diventa la somma, quindi il NE diventa esattamente caratterizzato dalla combinazione dei NE ottenuti su i problemi ortogonali

We denote $\bm{X}_{direc}, \ \bm{X}_{arbi}\in \R^M$ the 
inventories related to the directional and arbitrageur, respectively.
We refer to the previous setting as a \emph{Schied and Zhang multi-asset market impact game}, where the two agents are risk-neutrals and the market impact is constant $G_1>0$.
Thus, the following results hold.
\begin{pr}\label{pr_sZ_MIG}
In a Schied and Zhang multi-asset market-impact game where the two agents are a 
directional and an arbitrageur, and the market impact is constant, the Nash Equilibrium is time symmetric, i.e., 
\begin{align}\label{eq_symm_NE}
\bm{\xi}_{direc,k}^*&=\bm{\xi}_{direc,N+2-k}^*, \ k=1,2,\cdots,N+1,  \\
\bm{\xi}_{arbi,k}^*&=-\bm{\xi}_{arbi,N+2-k}^*, \ k=1,2,\cdots,N+1. 
\label{eq_symm_NE_2}
\end{align}
\end{pr}

In particular, the optimal schedule for agent $j$ at time step $k$ for the asset $i$ is provided by
$\xi_{j,i,k}=\sum_{l=1}^M v_{i,l}\cdot \xi_{j,l,k}^P$, 
where $v_{i,l}$ is the $i$-th element of the $l$-th eiegenvector of $Q$ and $\xi_{j,l,k}^P$ is the optimal schedule for the orthogonalized game where the cross impact is diagonal, corresponding to the eigenvalues of $Q$ for each asset, obtained by using the fundamental solutions
$\bm{v}_i$ and 
$\bm{w}_i$ computed using the decay kernel $G_1 \lambda_i$.
Even if the time symmetric property does not generally depend on the 
spectral decomposition of $Q$ and on the inventory of the fundamentalist, the property that characterizes the U-shape profile
of the optimal schedule might not be satisfied. Indeed, the convexity property may depend on the components of the particular eigenvector of $Q$.% {\color{blue}FC: Ti torna questo discorso?}

On the other hand, if 
the directional trader has inventory equal to one of the eigenvectors\footnote{In other words,
the directional trader wants to liquidate or buy a market factor following precise market signals,
where we interpret the eigenvectors of $Q$ as market factors.}
of $Q$, $\bm{v}_i$, then his/her inventory on the orthogonalized asset
is equal to the $i$-th element of the canonical base, i.e., 
the vector with one in position $i$ and zero otherwise.
This implies that with an exception of the orthogonalized asset 
$i$, the Nash equilibrium is zero, $\bm{\xi}^P_{direc,h}=\bm{0}$ for $h\neq i$, since the two agents have zero
(orthogonalized) inventories for $h\neq i$.
Therefore, for an asset $h$,
the optimal schedule for agent $j$ at time step $k$ can be simplified as
$\xi_{j,h,k}=\sum_{l=1}^M v_{h,l}\cdot \xi_{j,l,k}^P=
 v_{h,i}\cdot \xi_{j,i,k}^P
$, i.e., it is a rescaled version of the U-shape profile  
$\xi_{j,i,k}^P$ by the $h$-element of the $i$-th eigenvector of $Q$.
In particular, in this case we have the same evidence obtained for the one-asset case in Section \ref{sec_numerical_fit}, since the Nash equilibrium for each asset satisfies the relation \eqref{cond_linear_decay}.
% As an example we consider a primary market model
% with two asset, $M=2$ where the cross-impact matrix is given by 
% $$
% Q=\begin{bmatrix}
% 1 & 0.6\\ 0.6 & 1
% \end{bmatrix},
% $$
% $T=1$, $N=25$, $\theta=1$, $G_1=1$. 
% If the directional has inventory equal to $(1\ 1)^T$ then its Nash equilibrium has a U-shape, since $(1\ 1)^T$ is an eigenvector of $Q$. 

In conclusion, in the multi-asset case, when the directional trader liquidate a position proportional to one of the market factors 
represented by the eigenvectors of $Q$, the evidence of a transient market impact propagator function provided by the market impact game, when the price impact is set to a constant, still holds as for the one asset case.
We conclude by briefly discussing the general case of multi-agent
market impact game.

\subsection{The Multi-Agent Case}\label{sec_multi_agent}

{\color{blue}
Even if, in the previous setting, we may interpret  the two traders as representative agents, we now analyze the general setting with more than two agents.
}
If we consider a multi-asset primary market model with $J>2$ agents, we may use the results of \cite{luo_schied} and \cite{cordoni2020instabilities} to recover the related Nash equilibria of agents. However, even in the one asset case, the results of Section \ref{sec_ne_primary_model} are no more valid 
when we consider $J>2$ traders in the primary market model,
 since the fundamental solutions depend on the number of agents, which implies that the decay kernel matrix is no more Toeplitz in general, see e.g., \cite{luo_schied}. 
As an example, we consider $2$ arbitrageurs and a directional trader\footnote{All the agents are assumed to be risk-neutrals.}, where they trade the same asset.
Figure \ref{fig_3_agents_NE}
exhibits the related Nash equilibria for the agents when 
we set $T=1$, $N=25$, $G_1=1$, $\theta=1$. 
We observe that the solutions of the two arbitrageurs are identical.
Even if for the arbitrageur the optimal solution is 
always a round-trip strategy facing the same direction of the directional trader at the beginning of the session,
it is quite evident that the optimal solution for the directional is a U-shape which is no more time-symmetric. In particular, it is optimal for him/her 
to trade more at the end of session exploiting the impact of the arbitrageur.
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{plot_new/multi_agent_primary.eps}
    \caption{Nash equilibria for the primary market model with a directional trader and two arbitrageur, where 
    $T=1$, $N=25$, $G_1=1$, $\theta=1$. The solution of the two arbitrageurs are identical.}
    \label{fig_3_agents_NE}
\end{figure}

